Transformers are Provably Optimal In-context Estimators for Wireless Communications

Pre-trained transformers exhibit the capability of adapting to new tasks through in-context learning (ICL), where they efficiently utilize a limited set of prompts without explicit model optimization. The canonical communication problem of estimating transmitted symbols from received observations can be modeled as an in-context learning problem: received observations are a noisy function of transmitted symbols, and this function can be represented by an unknown parameter whose statistics depend on an unknown latent context. This problem, which we term in-context estimation (ICE), has significantly greater complexity than the extensively studied linear regression problem. The optimal solution to the ICE problem is a non-linear function of the underlying context. In this paper, we prove that, for a subclass of such problems, a single-layer softmax attention transformer (SAT) computes the optimal solution of the above estimation problem in the limit of large prompt length. We also prove that the optimal configuration of such a transformer is indeed the minimizer of the corresponding training loss. Further, we empirically demonstrate the proficiency of multi-layer transformers in efficiently solving broader in-context estimation problems. Through extensive simulations, we show that solving ICE problems using transformers significantly outperforms standard approaches. Moreover, just with a few context examples, it achieves the same performance as an estimator with perfect knowledge of the latent context. The code is available \href{https://github.com/vishnutez/in-context-estimation}{here}.

==> AISTATS-2025/contents-AISTATS/methodology.tex <==

\section{Methodology}

In this section, we describe the classical estimation techniques used to solve the estimation problem, along with a transformer model as an alternative.

\subsection{Context-aware and baseline estimators}
\label{baseline_genie_descriptions}
In this section, we describe some feasible context-aware estimators, that achieve a low MSE (close to that of \ref{eq:in_context_estimator}). For C1, $\theta = 0$, since the randomness of the channel parameter vector comes from a single random variable $\alpha$, the computation of the posterior mean involves an integral in one dimension. Hence, it can be computed in a computationally efficient manner. The exact expression appears in \ref{eq:one_ray_model_symbol_estimation}. 
In the remaining cases, we cannot evaluate the expression explicitly. In these cases, the context-aware estimator first computes the Linear Minimum Mean Square Estimate (LMMSE) $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$  of the channel parameter ${\vh}_{k+1}(\theta)$ given $S_k, \theta$. The exact details of computing the expression for $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$ are given in Appendix \ref{context_aware_estimators_derivation}. Incidentally, for $\theta=1$ in C1, and for all $\theta \in \Theta$ in C2, since $\vh_{k+1}(\theta)$ and $(\vy_t, t\in [k])$ are jointly Gaussian, conditioned on $(s_t, t\in[k])$, this channel estimate is in fact the minimum mean squared estimate (MMSE) of $\vh_{k+1}(\theta)$ given $S_k, \theta$. Then, the symbol is estimated by computing $\bE[s_{k+1} \mid \vh_{k+1}(\theta) = \hat{\vh}_{k+1}^{\rm LMMSE, \theta} \mid \vy_{k+1}]$; the exact expression for above conditional expectation is given in \ref{eq:symbol_estimate}.



For the context agnostic baseline, we describe an estimation procedure commonly used in the wireless communication. The estimator first computes the LMMSE of the channel (see Appendix \ref{baseline_for_agnostic_estimators}), which uses the correlation matrices corresponding to prior for the channel parameter process. Then, it estimates the symbol as the conditional mean, conditioned on the LMMSE for the channel. The exact details are given in Appendix \ref{baseline_for_agnostic_estimators}.

\subsection{Transformer} \label{training}
We train our transformer models as described in Section~\ref{in_context_estimation}. We follow the training setup used in \cite{ahuja2023incontext}, which is in turn based on the approach used in \cite{garg2023transformers}. For all experiments, we train a GPT-2 decoder-only model from scratch.

We specifically modify the setting in Section 4 of \cite{ahuja2023incontext}, regarding learning of functions sampled from a hierarchical distribution of function classes (``tasks"). In this setting, a task $\theta$ is sampled from some set of tasks $\Theta$, then a function $f$ is sampled from a set of functions $\mathcal{F}_\theta$ which is determined by $\theta$. In our case, $f$ is determined by the channel coefficients $\vh$, which we sample as described in Section~\ref{wireless_communication_problem}.

The training data is generated as follows. First we draw $\theta \sim {\rm Unif}(\Theta)$. In C1, we generate $\alpha \sim {\rm Unif}[0, \pi)$ and set $h^j_t(0) = \phi_j(\alpha)$. In C2, we generate the sequence $\vh^j = (h_t^j, t\in \bN)$ from a stationary Gaussian random process. For each training mini-batch, we re-sample $\theta$ and then independently sample each $\vh^j$.

As done in \cite{ahuja2023incontext}, we train our decoder models to perform prediction in the style of language models, where $$((\vy_1, \vx_1), (\vy_2, \vx_2), \dots, (\vy_k, \vx_k), \vy_{k+1})$$ are used to predict $\vx_{k+1}$. We use the sum of squared errors between all $(\vx_t, \hat{\vx}_t), t\in[k+1]$ as our loss function, where $\hat{\vx}_t =  T_W^{k+1}(S_k, \vy_{k+1})$. 

We set the number of antennae $d = 4$. For C2, we consider $M = 3$, where $v_1 = 5, v_2 = 15, v_3 = 30$ (all in m/s). These are representative of the typical values seen in practice for wireless communications. For C1, $\theta = 1$, we set $s = \lambda/4$. For C2, we use $f_c = 2.9 \times 10^9$ Hz, and $\lambda = f_c/c$, where $c = 3\times 10^8$ m/s is the speed of light. Further, we set the symbol duration $T_s =$ 1 millisecond in C2.

We include our model architecture details and other hyper-parameter settings in Appendix~\ref{parameters}.

==> AISTATS-2025/contents-AISTATS/related-work-old.tex <==

\section{Related Work}
\subsection{Transformers and In-Context Learning}
Transformer architectures have become a popular model architecture across a variety of problems. The recent popularity of this architecture is in large part due to the fact that multi-head self-attention units have been shown to perform well on a wide variety of natural language tasks~\cite{NIPS2017_3f5ee243}.

In \cite{LanguageModelsAreFewShotLearners} it was shown that GPT-3, a transformer-based large language model, is able to perform well on novel, unseen tasks in a few-shot or zero-shot manner, known as in-context learning. The authors of \cite{xie2022an} used synthetic data to show that in-context learning can be interpreted as Bayesian inference, wherein a model first attempts to infer the task and then uses this prediction to carry out the task.

\cite{garg2023transformers} and \cite{ahuja2023incontext} are closely related to our work. In \cite{garg2023transformers}, the authors explore in-context learning from a different perspective than prior work. Rather than looking at in-context learning in the natural language setting, they pose this as the problem of learning to perform least-squares estimation for linear regression by being trained on sequence data. The authors of \cite{ahuja2023incontext} build on this work and provide mathematical theory to describe how this can be interpreted as the model performing Bayesian inference by estimating a posterior distribution.

Other work has gone further in explaining the mechanisms by which transformers are able to perform in-context learning. Some authors have explored the behavior of simplified transformer models on synthetic linear regression problems, as compared to the globally optimal solutions for these problems\cite{mahankali2023step,Zhang2023TrainedTL}.
In \cite{whatlearningalgorithm}, it is shown by construction that transformers can learn to fit a linear model at inference time given a context. This tells us that, at least in theory, transformers can learn to literally perform regression and related computations given some data. A related line of work explores the manner by which transformer models carry out these optimization procedures and shows that transformer models can perform nontrivial gradient-based optimization procedures at inference time\cite{von2023transformers,ahn2023transformers}. 
In \cite{EmergentICL}, the authors test how properties of training data impact in-context learning behaviors. 
The authors of \cite{min2022rethinking} similarly study how the properties of the context itself impact in-context learning performance. 

In summary, many different research directions have provided ways to interpret and understand in-context learning and the mechanisms by which transformer models do it. In our work, we primarily use the Bayesian perspective to view this ability and to understand how we can apply it to the wireless communication domain.

\subsection{Machine Learning for Wireless Communication}
The problem of symbol estimation in the presence of an unknown channel is a canonical problem in wireless communication and there is a large body of literature that considers model-driven traditional signal processing approaches. 
When the prior distribution for the channel follows a hierarchical model with latent contexts such as what we study in this paper, optimal model-based estimators become computationally infeasible. 
While approximations to the optimal estimators have been studied with restricted priors, the structure and performance of such estimators are highly dependent on the priors.






Recently, there has been significant interest in using machine learning methods such as variational inference \cite{ChannelEstimationUsingVAE}, \cite{UnsupervisedEqualizationUsingVAEs} and deep neural network models such as fully connected neural networks \cite{DeepLearningAidedChannelEstimation}, convolutional neural networks \cite{LearningMMSEChannelEstimator}, and recurrent neural networks \cite{RNNforChannelEstimation} 
for channel estimation and for symbol estimation \cite{aoudia2021end}. The authors of \cite{faycal} design an  end-to-end wireless communication system design using learning-based approach.
The work of \cite{neumann} provides a principled way of designing channel estimators in the setting of wireless communication, by training CNN-based neural network to efficiently estimate the channel parameters when it follows a hierarchical prior. The authors of \cite{UnsupervisedLinearAndNonLinearChannelEqAndDecoding} used variational autoencoders (VAEs) and unsupervised learning to implicitly learn and decode symbols in a wireless channel. In \cite{SemisupervisedVAEForNonLinearChannels}, the authors use VAEs in a semi-supervised setting to operate over non-linear channels. The approach in \cite{deepLearningForTimeVaryingMIMOChannels} uses a long short-term memory (LSTM) based channel parameter estimator for a time-varying channel. They are interested in learning the spatial correlation structure of the channel coefficients across the receiver antennae.
 
 
 The main distinction of our work from the previous works is that we make the connection between the in-context learning capabilities of the transformer and the symbol estimation problem in wireless communication. We show how the problem fits naturally in the setting, and provide empirical evidence that transformers achieve near-optimal performance. A comparative study of the performance of the transformers and other machine learning models is left for the future work.

==> AISTATS-2025/contents-AISTATS/softmax-attention-theory.tex <==

\section{Main Results}
\label{sec:main_results}
In this section, we present our theoretical analysis for a single layer softmax attention transformer (SAT) as an estimator for the problem corresponding to \eqref{eq:complex-est-prob}.
We work with the following assumption.
\begin{assumption}
\label{assum:SIMO-model} The distributions of the hidden process, input symbols, and noise are characterized as follows.
\begin{enumerate}[label=(\alph*)]
    \item The hidden process is time invariant, i.e., $\tilde{\vh}_t(\theta) = \tilde{\vh}(\theta)$, where $\tilde{\vh}(\theta) \sim \bP_{h\mid \theta}$ is a \emph{fixed} hidden variable under the context $\theta \sim \bP_\Theta$.
    \item The inputs $\tilde{x}_t \stackrel{\rm iid}{\sim} \bP_x$ where $\bP_x$ is some distribution on $\tilde{\cX}$, and $\tilde{\cX} \subset \bC$ is a finite subset of the unit circle in $\bC$, i.e., $\abs{z} = 1$ for any $z \in \tilde{\cX}$. 
    \item The noise samples $\tilde{\vz}_t \stackrel{\rm iid}{\sim} \cC\cN(\0, \tilde{\bSigma}_{z})$ for some real positive definite matrix $\tilde{\bSigma}_z \in \bR^{d\times d}$.
\end{enumerate}
\end{assumption}

Then, the real equations are given by
\begin{equation}
\label{eq:real-constant-h}
    \vy_t = \mH(\theta) \vx_t + \vz_t, \quad t\ge 1
\end{equation}
 where $\vz_t \sim \cN(\0, \bSigma_z)$ such that $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
    \tilde{\bSigma}_z & \0 \\
    \0 &  \tilde{\bSigma}_z
\end{bmatrix}$, and note that $\bSigma_z^{-1} = 2 \begin{bmatrix}
    \tilde{\bSigma}_{z}^{-1} & \0 \\
    \0 &  \tilde{\bSigma}_{z}^{-1}
\end{bmatrix}$, and $\vx_t \in \cX$ can be identified as a subset of unit sphere $\bS^2$ in $\bR^2$. From now on, we only work with the above real quantities. 

We next derive the minimum mean squared error (MMSE) estimate for $\vx_t$ given $\vy_t$ and $\mH_t = \mH$.
Note that when $\mH_t = \mH$ is known, the dependence of the estimation problem on $\theta$ vanishes.
Further, $\left\{ (\vy_t, \vx_t) \right\}$ are conditionally independent and identically distributed (iid) given $\mH_t = \mH$ for all $t$. Therefore, the MMSE estimation corresponds to estimating $\vx$ from $\vy = \mH \vx + \vz$ when $\mH$ is known.

\begin{lemma}
\label{lem:opt-MMSE-PSK}
{\bf (MMSE estimate)}
    The optimal estimator $\hat{\vx}^{\rm MMSE}: \bR^{2d} \times \bR^{2d\times 2} \to \bR^2$ for $\vx \in  \cX \subset \bS^2$ given $\vy \in \bR^{2d}, \mH \in \bR^{2d\times 2}$ where $\vy = \mH \vx + \vz$ for some $\vz \sim \cN(\0, \bSigma_z)$ is given by
    \begin{align*}
        \hat{\vx}^{\rm MMSE}(\vy, \mH; \bSigma_z, \bP_x) = \bE[\vx \mid \vy, \mH] = \frac{\sum_{\vx \in \cX}\vx \bP_x(\vx) \exp(\vy^T \bSigma_z^{-1} \mH \vx)}{\sum_{\vx \in \cX}  \bP_x(\vx) \exp(\vy^T \bSigma_z^{-1} \mH \vx)},
    \end{align*}
    where $\mH \triangleq \begin{bmatrix}
        \operatorname{Re}(\tilde{\vh}) & -\operatorname{Im}(\tilde{\vh}) \\
        \operatorname{Im}(\tilde{\vh}) & \operatorname{Re}(\tilde{\vh})
    \end{bmatrix}$ for some $\tilde{\vh} \in \bC^d$, and $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
        \tilde{\bSigma}_z & \0 \\
        \0 & \tilde{\bSigma}_z
    \end{bmatrix}$ for some symmetric positive definite matrix $\tilde{\bSigma}_z \in \bR^{d\times d}$.
\end{lemma}

\proof{This follows from elementary computations involving Bayes theorem (see Appendix~\ref{sec:appendix-finite-estimation}).}

Since $\mH(\theta)$ is not known in the problems we consider, the above estimator essentially provides a lower bound on the performance of any in-context estimator. 

Let us consider a single layer softmax attention transformer (SAT) to solve the in-context estimation of $\vx$ given observation $\vy$ and $n$ in-context examples $\cP^n_\theta \triangleq \{(\vy_t, \vx_t), t\in[n]\}$, where $(\vy, \vx)$ and $(\vy_t, \vx_t)$ in $\cP_\theta^n$ satisfy \eqref{eq:real-constant-h}. 
Let $\mT^{\rm SA}$ denote an SAT with the query, key, and value matrices $\tilde{\mW}_Q, \tilde{\mW}_K, \tilde{\mW}_V$ respectively, acting on $(n+1)$ tokens $\vu_t \triangleq [\vy_t^T~\vx_t^T]^T \in \bR^{2d+2}$ for $t\in[n]$ and $\vu_{n+1} \triangleq [\vy^T~\0_2^T]^T \in \bR^{2d+2}$. Let $\mU_{n+1}$ be the matrix with columns $\vu_t$ for $t\in[n+1]$. Then, the $(n+1)$th output token is given by
\begin{align}
\label{eq:transformer-output}
    \mT_{n+1}^{\rm SA}(\mU_{n+1}) = \frac{\sum_{t=1}^{n+1} \tilde{\mW}_V \vu_t \exp(\vu_{n+1}\tilde{\mW}_Q^T \tilde{\mW}_K \vu_t)}{\sum_{t=1}^{n+1} \exp(\vu_{n+1}\tilde{\mW}_Q^T \tilde{\mW}_K \vu_t)}.
\end{align}

% The estimate of the above SAT for $\vx$ is provided by the last two entries in the $(n+1)$th output token, i.e., $[\mT_{n+1}^{\rm SA}]_{2d+1:2d+2}$. We denote this estimate with $n$ examples as $\hat{\vx}_{\rm SA}^n$.

The estimate of the SAT for \(\vx\) using \(n\) examples, denoted by \(\hat{\vx}^{\rm SA}_{n}\)  is obtained from the last two elements of the \((n+1)\)th output token, i.e., \([\mT_{n+1}^{\rm SA}]_{2d+1:2d+2}\).
Thus, the first $n$ columns of $\tilde{\mW}_V$ do not affect the output $\hat{\vx}^{\rm SA}_{n}$, hence we set them to zeros without loss of generality. Motivated by the form of the MMSE estimate, we choose to re-parameterize the remaining entries of the weights as below:
\begin{align}
\label{eq:query-key-values}
    \tilde{\mW}_Q &= \begin{bmatrix} \mW_Q & \0_{2d\times 1} \\ \0_{1\times 2d} & \0_{2\times 2}\end{bmatrix}, \quad \tilde{\mW}_K = \begin{bmatrix} \mW_K & \0_{2d\times 1} \\ \0_{1\times 2d} & \0_{2\times 2}\end{bmatrix}, \\
    \tilde{\mW}_V &= \begin{bmatrix}
    \0_{2d\times 2d} & \0_{2d\times 1} \\ \0_{1\times 2d} & \mI_2
\end{bmatrix}.
\end{align}

Denoting $\mW \triangleq \mW_{\rm Q}^T \mW_{\rm K} \in \bR^{2d\times 2d}$, using \eqref{eq:query-key-values} in \eqref{eq:transformer-output}, we get
\begin{align*}
    \hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW) = \frac{\sum_{t=1}^n \vx_t \exp(\vy^T \mW \vy_t) }{\exp(\vy^T \mW \vy) + \sum_{t=1}^{n} \exp(\vy^T \mW \vy_t)}.
\end{align*}

\begin{lemma}
\label{lem:convergence-SA-PSK}
{\bf (Functional form of asymptotic softmax attention)}
For any $\theta \in \Theta$, suppose $\mH_i(\theta) = \mH$ is the common hidden parameter for $i \in [n+1]$, such that $\vy_i = \mH \vx_i + \vz_i$, and $\vy = \mH \vx + \vz$.
For a prompt $\mU_{n+1}$ with the $t$th column constructed as 
$\vu_t \triangleq [\vy_t^T, \vx_t^T]^T$ for $t\in[n]$ and $\vu_{n+1} \triangleq [\vy^T, \0_2^T]^T$, the estimated value by the transformer $\hat{\vx}_n^{\rm SA}$ with parameter $\mW$ satisfies
\begin{align*}
    \lim_{n \to \infty} \hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW) = \frac{\sum_{\vx \in \cX}\vx  \bP_x(\vx) \exp(\vy^T \mW \mH \vx)}{\sum_{\vx \in \cX}  \bP_x(\vx) \exp(\vy^T \mW \mH \vx)} ~{\rm a.s.}
\end{align*}
\end{lemma}

\proof{This follows by a careful application of the strong law of large numbers (see Appendix \ref{sec:appendix-finite-estimation}).}

\begin{theorem}
{\bf (Existence of a softmax attention estimator that is asymptotically optimal)} 
\label{thm:opt-SA-PSK}
%There exists a softmax attention transformer such that it is asymptotically an optimal estimator in the mean squared error sense, i.e., a.s.
There exists a softmax attention transformer such that, for any asymptotically long prompt, its estimate converges to the optimal MMSE estimator, i.e.,
\begin{align*}
     \lim_{n \to \infty} \hat{\vx}^{\rm SA}_{n}(\cdot; \bSigma_z^{-1}) = \hat{\vx}^{\rm MMSE}(\cdot; \bSigma_z, \bP_x) \quad \text{a.s.}
\end{align*}
\end{theorem}
\proof{This result follows directly from Lemma \ref{lem:opt-MMSE-PSK} and Lemma \ref{lem:convergence-SA-PSK}.}

This establishes the fact that the single layer softmax attention transformer architecture is expressive enough to asymptotically achieve optimal performance.

We then turn to the training process: can the training of such a transformer with (asymptotically) long prompt length achieve optimal performance?

To begin answering this question, we define the training procedure as follows.
Let prompt $j\in [n_p]$ in the training data be $\mU^j_{n+1}$ with columns $[\vu_1^j, \vu_2^j, \dots, \vu_n^j, \vu^j]$; therein, $\vu_i^j = [(\vy_i^j)^T~(\vx_i^j)^T]^T$, $\vu^j = [(\vy^j)^T~(\vx^j)^T]^T \in \bR^{2d+2}$, $\vy_i^j = \mH^j \vx_i^j + \vz_i^j$, where $\vz^j, \vz_i^j \stackrel{\rm iid}{\sim} \cN(\0,\bSigma_z)$, $\vx^j, \vx_i^j \stackrel{\rm iid}{\sim} \bP_x(\cX)$, and $\mH^j \in \bR^{2d\times 2}$ is constructed from $\tilde{\vh}$ chosen from a distribution $\bP_{h\mid \theta}$ for some $\theta \sim \bP_\Theta$.

Let us define the pre-training loss of the transformer as
\begin{equation*}
    \cL_n^{n_p}(\mW) \triangleq \textstyle \frac{1}{n_p} \sum_{j=1}^{n_p} \norm{\hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW)-\vx^j}_2^2 .
\end{equation*}
We define the population loss as $\cL_n(\mW) \triangleq \lim_{n_p\to \infty} \cL_n^{n_p}(\mW)$. Thus, by the strong law of large numbers, $\cL_n(\mW) = \bE_{\theta \sim \bP_\Theta, \tilde{\vh} \sim \bP_{h\mid \theta}, \vz\sim\cN(\0, \bSigma_z), \vx, \vx_i \sim \bP_x}[\norm{\hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW)-\vx}_2^2]$ a.s., where the expectation is over the prompts in the pre-training distribution. We write the loss as $\cL_n(\mW; \bSigma_z, \bP_x, \bP_{\Theta,h})$ to indicate the dependence on the distribution of $\vh$, the input set $\cX$, and $\bSigma_z$ during the training. Finally, we define the asymptotic loss in the limit as $n\to\infty$ as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$, and write $\cL(\mW; \bSigma_z, \bP_x, \bP_{\Theta,h})$.

\begin{theorem}
{\bf (Global minimizer)}
\label{thm:global-min-PSK} For any pre-training distribution $\bP_{\Theta, h}$ on the latent context of the hidden parameters, and any distribution of the inputs $\bP_x$, the matrix $\bSigma_z^{-1} \in \bR^{2d\times 2d}$ is the global minimizer of $\cL(\cdot; \bSigma_z, \bP_x, \bP_{\Theta,h})$.
\end{theorem}
\proof{It follows from the properties of conditional expectation, the uniform boundedness (in $n$) of $\hat{\vx}^{\rm SA}_{n}(\cdot; \mW)$, and the dominated convergence theorem (see Appendix \ref{sec:appendix-finite-estimation}).}

We remark that the optimality in Theorem \ref{thm:opt-SA-PSK} and Theorem \ref{thm:global-min-PSK} is only in the asymptotic limit. As such, the results are about the expressiveness and the minimizer of the training loss for a softmax attention transformer, akin to the results of linear attention in \cite{zhang2024trained} (barring convergence of the training procedure). Typically, we are interested in optimal algorithms given $n$ examples. For optimal estimators in the case of finite context length, the dependence on $\theta$ becomes important. To exploit this dependence, we next introduce multi-layer transformers as viable in-context estimators and demonstrate their effectiveness. 


==> AISTATS-2025/contents-AISTATS/softmax-for-BPSK.tex <==
\section{Softmax Attention}

\begin{problem}
{\bf (In-context estimation)}
\label{pr:ice}
    Estimate $x$ from $\vy = \vh x + \bepsilon$ and $n$ in-context examples (pilots) $\{(\vy_i, x_i)\}_1^n$ that satisfy $\vy_i = \vh x_i + \bepsilon_i$ where $\vh \in \bR^d$ is a fixed hidden variable (channel) and  $\bepsilon, \bepsilon_i \stackrel{\rm iid}{\sim} \cN(\0, \bSigma_{\bepsilon})$, $x, x_i \stackrel{\rm iid}{\sim} \cU\{\pm 1\}$.
\end{problem}

First, we derive the minimum mean squared error (MMSE) estimate for $x$ given $\vy$ and the hidden variable $\vh$.

\begin{lemma}
\label{lem:opt-MMSE}
{\bf (MMSE estimate)}
    The optimal estimator $\hat{x}_{\rm MMSE}: \bR^d \times \bR^d \to \bR$ for the transmitted symbol $x$ given $\vy, \vh$ where $\vy = \vh x + \bepsilon$ for some $\bepsilon \sim \cN(\0, \bSigma_{\bepsilon})$ is given by
    \begin{align*}
        \hat{x}_{\rm MMSE}(\vy, \vh; \bSigma_{\bepsilon}) = \bE_{x, \bepsilon}[x \mid \vy, \vh] = \tanh(\vy^T\bSigma_{\bepsilon}^{-1}\vh).
    \end{align*}
\end{lemma}
\proof{It follows from elementary computations involving Bayes theorem (see Appendix \ref{sec:appendix}). }

Note that the above estimator assumes that the channel is perfectly known to the estimator. Unlike the linear regression problem, even if the hidden variable is known to the estimator, the estimate for $x$ is still not perfect, in the sense that the estimation error is non-zero. We next consider a transformer to solve the above problem when $\vh$ is not known. Specifically, let $T^{\rm SA}$ be a single layer softmax attention (SA) transformer $T$ with the query, key matrices of the form $\tilde{\mW}_s = \begin{bmatrix} \mW_s & \0 \\ \0 & 0\end{bmatrix}$, $s = {\rm Q}, {\rm K}$, and the value matrix $\tilde{\mW}_{\rm V} = \begin{bmatrix}
    \0 & \0 \\ \0 & 1
\end{bmatrix}$, acting on tokens $\vt_i \triangleq [\vy_i^T~x_i]^T \in \bR^{d+1}$ for $i\in[n]$ and $\vt \triangleq [\vy^T~0]^T \in \bR^{d+1}$.  Denoting $\mW \triangleq \mW_{\rm Q}^T \mW_{\rm K}$, we can write the predicted value of $x$ by the transformer as
\begin{align*}
    T^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n; \mW) = \frac{\sum_{i=1}^n x_i \exp(\vy^T \mW \vy_i) }{\exp(\vy^T \mW \vy) + \sum_{i=1}^{n} \exp(\vy^T \mW \vy_i)}.
\end{align*}


\begin{lemma}
\label{lem:convergence-SA}
{\bf (Functional form of asymptotic softmax attention)} For $i\in [n]$, if $x_i, \vy_i$ are such that $\vy_i = \vh x_i + \bepsilon_i$, and $\vy = \vh x + \bepsilon$, then we have
\begin{align*}
    \lim_{n \to \infty} T^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n;  \mW) = \tanh(\vy^T \mW \vh)~{\rm a.s.}
\end{align*}
\end{lemma}

\proof{It follows by a careful application of the strong law of large numbers (see Appendix \ref{sec:appendix}).}

\begin{theorem}
{\bf (Existence of a softmax attention estimator that is asymptotically optimal)} 
\label{thm:opt-SA}
There exists a softmax attention transformer such that it is asymptotically an optimal estimator in the mean squared error sense, i.e.,
\begin{align*}
    \lim_{n\to \infty} T_n^{\rm SA}(\cdot; \bSigma_{\bepsilon}^{-1}) = \hat{x}_{\rm MMSE}(\cdot; \bSigma_{\bepsilon})
\end{align*}
\end{theorem}
\proof{It directly follows from Lemma \ref{lem:opt-MMSE} and Lemma \ref{lem:convergence-SA}.}

Now that we proved existence, can the training such a transformer with $n\to\infty$ achieve the above optimal estimate?


In order to answer the above question, we first define a training procedure as follows. Denote the $j$th prompt in the training data as $[\vt_1^j, \vt_2^j, \dots, \vt_n^j, \vt^j]$  for $j\in [p]$ such that $\vt_i^j = [(\vy_i^j)^T~x_i^j]^T, \vt=[(\vy^j)^T~x^j]^T \in \bR^{d+1}, \vy_i^j = \vh^j \vx_i^j + \bepsilon_i^j$, where $\bepsilon^j, \bepsilon_i^j \stackrel{\rm iid}{\sim} \bSigma_{\bepsilon}, x^j, x_i^j \stackrel{\rm iid}{\sim} \cU\{\pm 1\}$ and $\vh^j \in \bR^d$ can be chosen from a distribution $\mu_\vh$.


Let us define the pre-training loss of the transformer with the above training procedure as $\cL_n^p(\mW) \triangleq \frac{1}{p} \sum_{j=1}^p (T_n^{\rm SA}(\vy^j, \{\vy_i^j\}_{i=1}^n, \{x_i^j\}_{i=1}^n; \mW)-x^j)^2$. We define the population loss as $\cL_n(\mW) \triangleq \lim_{p\to \infty} \cL_n^p(\mW)$. Thus, by the strong law of large numbers, $\cL_n(\mW) = \bE_{\vh\sim\mu_{\vh}, \bepsilon \sim \cN(\0, \bSigma_{\bepsilon}), x, x_i \sim \cU\{\pm 1\}}[(T_n^{\rm SA}(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n; \mW)-x)^2]$ a.s., where the expectation is over the prompts in the pre-training distribution. We write the loss as $\cL_n(\mW; \mu_\vh, \bSigma_{\epsilon})$ to indicate the dependence on the distribution of $\vh$ and $\bepsilon$ during the training. Finally, we define the asymptotic loss in the limit as $n\to\infty$ as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$, and write $\cL(\mW;\mu_\vh, \bSigma_{\bepsilon})$. Then, we have the following result.
\begin{theorem}
{\bf (Global minimizer)}
\label{thm:global-min} For any $\mu_\vh$, $\mW^* = \bSigma_{\bepsilon}^{-1}$ is the global minimizer of $\cL(\cdot; \mu_\vh, \bSigma_{\bepsilon})$.
\end{theorem}
\proof{It follows from the properties of conditional expectation, the uniform boundedness (in $n$) of $T_n^{\rm SA}(\cdot; \mW)$, and the dominated convergence theorem (see Appendix \ref{sec:appendix}).}





% \subsection{Convergence of estimate by softmax attention to conditional mean estimate}

% Let $P(y=+1) = P(y=-1) = 1/2$. Given $\vh$, the MMSE estimate of $y$ from $\vx = \vh y + \vz$ where $\vz \sim \cN(0,\bSigma)$ is given  the conditional mean estimate (CME) as
% \begin{align*}
%     y^{\rm CME}(\vx,\vh;\bSigma) = \bE[y \mid \vx, \vh] 
%     &= P(y=1 \mid \vx,\vh)-P(y=-1 \mid \vx,\vh) \\
%     &= \frac{P(y=1) P(\vx,\vh \mid y=1)}{P(\vx,\vh)} -\frac{P(y=-1) P(\vx,\vh \mid y=-1)}{P(\vx,\vh)} \\
%     &= \frac{ P(y=+1) P(\vx, \vh \mid y=1) - P(y=-1) P(\vx, \vh \mid y=-1)}{ P(y=+1) P(\vx, \vh \mid y=1) + P(y=-1) P(\vx, \vh \mid y=-1)} \\
%     &= \frac{P(\vz = \vx-\vh) - P(\vz=\vx+\vh)}{P(\vz = \vx-\vh) + P(\vz=\vx+\vh)} \\
%     &= \frac{\exp(-\frac{1}{2}(\vx-\vh)^T \bSigma^{-1}(\vx-\vh))-\exp(-\frac{1}{2}(\vx+\vh)^T \bSigma^{-1}(\vx+\vh))}{\exp(-\frac{1}{2}(\vx-\vh)^T \bSigma^{-1}(\vx-\vh))+\exp(-\frac{1}{2}(\vx+\vh)^T \bSigma^{-1}(\vx+\vh))} \\
%     &= \frac{1-\exp(-\frac{1}{2} ((\vx+\vh)^T \bSigma^{-1}(\vx+\vh)-(\vx-\vh)^T \bSigma^{-1}(\vx-\vh)))}{1+\exp(-\frac{1}{2} ((\vx+\vh)^T \bSigma^{-1}(\vx+\vh)-(\vx-\vh)^T \bSigma^{-1}(\vx-\vh)))} \\
%     &= \frac{1-\exp(-\frac{1}{2}(4\vx^T\bSigma^{-1}\vh))}{1+\exp(-\frac{1}{2}(4\vx^T\bSigma^{-1}\vh))} = \tanh(\vx^T\bSigma^{-1}\vh) = \frac{\exp(\vx^T\bSigma^{-1}\vh)-\exp(-\vx^T\bSigma^{-1}\vh)}{\exp(\vx^T\bSigma^{-1}\vh)+\exp(-\vx^T\bSigma^{-1}\vh)}.
% \end{align*}

% \subsubsection{Under balanced inputs in the prompt}
% For the softmax attention, for the ease of notation we denote $\vx_{N+1}$ as $\vx$ and $y_{N+1}$ as $y$. For $N=2n$ assume that we have balanced inputs, i.e., $y_i = +y$ and $y_{n+i} = -y$ for $i\in[n]$. Hence, we have $\vx_i = \vh y + \vz_{i}, \vx_{n+i} = -\vh y + \vz_{n+i}$, for $i\in[n]$. Then, for $\mW = \bSigma^{-1}$ we can write the output of the softmax attention as
% \begin{align*}
%     &y^{\rm SA}_{n}(\vx,\{y_i\},\{\vx_i\}; \mW) \triangleq y \frac{\sum_{i=1}^n \exp(\vx^T\mW\vx_i) - \sum_{i=1}^n \exp(\vx^T \mW\vx_{n+i})}{\exp(\vx^T\mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW\vx_i) + \sum_{i=1}^n \exp(\vx^T \mW\vx_{n+i})} \\
%     &\hspace{2pt} = y\frac{\frac{1}{n} \sum_{i=1}^n \exp((\vx^T\mW(\vh y +\vz_i))) - \frac{1}{n}\sum_{i=1}^n \exp((\vx^T\mW(-\vh y +\vz_{n+i}))}{ \frac{1}{n}\exp(\vx^T\mW \vx) + \frac{1}{n} \sum_{i=1}^n \exp((\vx^T\mW(\vh y +\vz_i))) + \frac{1}{n}\sum_{i=1}^n \exp((\vx^T\mW(-\vh y +\vz_i)))} \\
%     &\hspace{2pt} = y\frac{\exp(\vx^T\mW\vh y)(\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_i)) - \exp(-\vx^T\mW\vh y) (\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW^{-1}\vz_{n+i}))}{\frac{1}{n}\exp(\vx^T\mW\vx)+\exp(\vx^T\mW\vh y)(\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_i)) + \exp(-\vx^T\mW\vh y) (\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_{n+i}))}.
% \end{align*}
% For any given $\vx,\vh \in \bR^d$ (denote $\bE[\cdot \mid \vx]$ as $\bE[\cdot]$), $\xi_j \triangleq \vx^T \mW\vz_j = 0$ are iid Gaussian random variables with mean $\bE[\xi_1]  = \vx^T\mW\bE[\vz_1] = 0$, and variance $\bE[\vx^T \mW \vz_1 \vz_1^T \mW^T \vx] = \vx^T \mW\bSigma\mW^T\vx \triangleq \gamma(\vx)$. We call $\gamma(\vx)$ the instantaneous SNR. Hence, $\xi_j \stackrel{\rm iid}{\sim}  \cN (0, \gamma(\vx))$, $j\ge 1$. Therefore, $\zeta_j \triangleq \exp(\xi_j)$ are iid log-normal random variables with parameters $\mu_0 \triangleq 0, \sigma_0^2 \triangleq \gamma(\vx)$ with mean and variance given by $\bE[\zeta_1] = \exp(\mu_0 + \sigma_0^2/2) = \exp(\gamma(\vx)/2)$, and ${\rm Var}(\zeta_1) = (\exp(\sigma_0^2)-1)\exp(2\mu_0 + \sigma_0^2) = (\exp(\gamma(\vx))-1)\exp(\gamma(\vx)) < \infty$. Hence, by the strong law of large numbers $\frac{1}{n}\sum_{i=1}^n \zeta_i \to \bE[\zeta_1]$ a.s. Therefore, by continuity, for any $\vx,\{y_i\}, \{\vx_i\}$, we get $y^{\rm SA}_{n}(\vx,\{y_i\},\{\vx_i\}; \mW) \to y \frac{\bE[\zeta_1]\exp(\vx^T\mW\vh)-\bE[\zeta_1]\exp(-\vx^T\mW\vh)}{\bE[\zeta_1]\exp(\vx^T\mW\vh)+\bE[\zeta_1]\exp(-\vx^T\mW\vh)} = \frac{\exp(\vx^T\mW\vh)-\exp(-\vx^T\mW\vh)}{\exp(\vx^T\mW\vh)+\exp(-\vx^T\mW\vh)} \triangleq \tanh(\vx^T\mW\vh)$ a.s. for any $\bSigma \succ 0, \vh,\vx\in\bR^d$.
% When $n$ is large, then the output of the transformer is ${y}^{\rm SA}(\cdot; \mW) = \tanh(\vx^T\mW\vh) = y^{\rm CME}(\cdot ; \mW)$.

% \subsubsection{Arbitrary inputs}

% Let $\{y_i\}_1^n \stackrel{\rm iid}{\sim} {\rm Unif}(\pm 1), \{\vz_i\}_1^n \stackrel{\rm iid}{\sim} \cN(\0, \bSigma)$, and $\vx_i = \vh y_i + \vz_i$ for $i\in[n]$. Denote $I_n^+ \triangleq \{i \in [n]: y_i = y\}$, and $I_n^{-} \triangleq [n] \setminus I_n^{+}$. Then, the output of the softmax attention can be written as
% \begin{align*}
%     &y_n^{\rm SA}(\vx,\{\vx_i\}_1^n,\{y_i\}_1^n;\mW)
%     = \frac{\sum_{i=1}^n y_i \exp(\vx^T \mW \vx_i)}{\exp(\vx^T \mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW \vx_i)} \\
%     &= y\frac{\exp(\vx^T\mW \vh y) \frac{\abs{I_n^+}}{n} \frac{1}{\abs{I_n^{+}}}\sum_{i\in I_n^{+}} \exp(\vx^T\mW \vz_i) -  \exp(-\vx^T\mW \vh y) \frac{\abs{I_n^-}}{n} \frac{1}{\abs{I_n^{-}}} \sum_{i\in I_n^{-}} \exp(\vx^T \mW \vz_i)}{\frac{1}{n}\exp(\vx^T \mW \vx) + \frac{\abs{I_n^+}}{n} \frac{1}{\abs{I_n^{+}}} \exp(\vx^T\mW \vh y) \sum_{i\in I_n^{+}} \exp(\vx^T\mW \vz_i) + \frac{\abs{I_n^-}}{n} \frac{1}{\abs{I_n^{-}}} \exp(-\vx^T\mW \vh y)\sum_{i\in I_n^{-}} \exp(\vx^T \mW \vz_i)}
% \end{align*}
% By the strong law of large numbers, $\abs{I_n^+}, \abs{I_n^-} \to \infty$ and $\frac{\abs{I_n^+}}{n},\frac{\abs{I_n^-}}{n} \to \frac{1}{2}$ a.s. Further,
% \begin{align*}
%     \frac{1}{\abs{I_n^+}} \sum_{i \in I_n^+} \exp(\vx^T \mW \vz_i), \frac{1}{\abs{I_n^-}} \sum_{i \in I_n^-} \exp(\vx^T \mW \vz_i) \to \bE[\exp(\vx^T\mW \vz_1)])~{\rm a.s.},
% \end{align*}
% and so we get by continuity, $y_n^{\rm SA}(\vx,\{\vx_i\}_1^n,\{y_i\}_1^n;\mW) \to \tanh(\vx^T\mW \vh)  = y^{\rm CME}(\vx,\vh; \mW)$ a.s.

% % For $n$ \emph{large}, this is the optimal thing to do. But, what happens when $n$ is small? The transformer might do some bias variance kind of trade off to fit $\mW$.

% We ask the following questions:
% \begin{enumerate}[label=(\roman*)]
%     \item With the intuition that $y^{\rm CME}$ is the best estimate given $\vh$, and plugging $\mW = \bSigma^{-1}$ a softmax attention layer would implement it, is $\mW^* = \bSigma^{-1}$ the global minimizer of $\cL$?
%     \item If we start we arbitrary $\mW^0$ as perform gradient descent in the large context limit ($N$ large), then can we guarantee $\mW^{k} \to \bSigma^{-1}$ as $k\to \infty$?
%     \item What happens when there are two types of noise in the training data $\vz^{(1)} \sim \cN(\0, \bSigma_1)$ and $\vz^{(2)}\sim \cN(\0, \bSigma_2)$?
% \end{enumerate}



% \subsection{Global minimizer of the asymptotic loss}

% In this section, we answer (i) in the affirmative. Denote $\cL_n(\mW) \triangleq \bE[(y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)-y)^2]$, and consider the loss in the limit as $n\to\infty$ defined as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$. We want to show that $\mW^* = \bSigma^{-1}$ is the minimizer of $\cL$.

% We know from the previous section that $\lim_{n\to \infty} y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW) = y^{\rm CME}(\mW)$ a.s. Now, since
% \begin{align*}
%     \abs{y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)} &= \Big| \frac{\sum_{i=1}^n y_i \exp(\vx^T \mW \vx_i)}{\exp(\vx^T \mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW \vx_i)} \Big| \le \frac{\sum_{i=1}^n \abs{y_i} \exp(\vx^T \mW \vx_i)}{\sum_{i=1}^n \exp(\vx^T \mW \vx_i)} = 1,
% \end{align*}
% we have that $\forall \mW \in \bR^{d\times d}, \forall n\ge 0$, $0\le g_n(\mW) \triangleq (y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)-y)^2 \le 4$. Therefore, $\{g_n(\mW)\}_1^\infty$ are bounded, integrable random variables. Thus, using the bounded convergence theorem, we get
% \begin{align*}
%     \cL(\mW) \triangleq \limsup_{n\to \infty}\bE[g_n(\mW)] = \bE[\limsup_{n\to\infty} g_n(\mW)] &= \bE[(\limsup_{n\to\infty}y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW) -y)^2] \\
%     &=\bE[(y^{\rm CME}(\mW)-y)^2] \triangleq \delta(\mW).
% \end{align*}

% Consider the problem $\min_{\hat{y}_n \in \cY_n} \bE[(\hat{y}_n-y)^2]$, where $\cY_n \triangleq \{f \in L^2: f ~{\rm is}~\sigma(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n, \vh){\rm-measurable}\}$. Then, the minimizer is the conditional expectation given by
% \begin{align*}
%     \hat{y}^*(\vx, \{\vx_i\}_1^{n}, \{y_i\}_1^n, \vh) &= \bE[y \mid \vx, \{\vx_i\}_1^{n}, \{y_i\}_1^n, \vh] = \bE[y \mid \vx, \vh] = \tanh(\vx^T \bSigma^{-1}\vh) \triangleq y^{\rm CME}(\bSigma^{-1}),
% \end{align*}
% and the minimum value is $\bE[(y^{\rm CME}(\bSigma^{-1})-y)^2] = \delta(\bSigma^{-1})$. 
% Thus, we just showed that $\forall n \ge 0,\forall \hat{y}_n \in \cY_n$, we have $\bE[(\hat{y}_n-y)^2] \ge \delta(\bSigma^{-1})$. In particular, $\forall \mW \in \bR^{d\times d}$, $\forall n \ge 0$ since $y_n^{\rm SA}(\cdot ;\mW) \in \cY_n$, we have $\cL_n(\mW) \ge \delta(\bSigma^{-1})$. Therefore, for any $\mW \in \bR^{d\times d}$, we get $\cL(\mW) = \limsup_{n\to \infty} \cL_n(\mW) \ge \delta(\bSigma^{-1}) = \cL(\bSigma^{-1})$, whence $\mW^* \triangleq \bSigma^{-1}$ is the global minimizer of $\cL$.

% \subsection{Convergence of the gradient descent}


% In this section, we \emph{try} to show that (ii) is true (not much of a success). Let $\mu$ be the distribution of $\vh$. From the previous section, we have that
% \begin{align*}
%     \cL(\mW) = \delta(\mW) &= \bE[(\tanh(\vx^T \mW \vh)-y)^2] \\
%     &= \bE_{y, \vh, \vz}[(\tanh((y\vh^T+\vz^T)\mW \vh)-y)^2].
% \end{align*}
% We have that 
% \begin{align*}
%     \phi_\vh(y) &\triangleq \bE_{\vz}[(\tanh((y\vh^T+\vz^T)\mW \vh)-y)^2] \\
%     &= \bE_{\vz}[(-\tanh((-y\vh^T-\vz^T)\mW \vh)-y)^2] \\
%     &= \bE_{\vz}[(\tanh((-y\vh^T-\vz^T)\mW \vh)-(-y))^2] \\
%     &= \bE_{\tilde{\vz} \triangleq -\vz}[(\tanh((-y\vh^T+\tilde{\vz}^T)\mW \vh)-(-y))^2] \\
%     &= \bE_{\vz}[(\tanh(((-y)\vh^T+\vz^T)\mW \vh)-(-y))^2] = \phi_\vh(-y).
% \end{align*}
% Thus, we get
% \begin{align*}
%     \cL_\mu(\mW) = \bE_{y, \vh\sim \mu}[\phi_\vh(y)] = P(y=1)\bE_\vh [\phi_\vh(1)]+P(y=-1)\bE_\vh [\phi_\vh(-1)] = \frac{1}{2} \bE_{\vh}[\phi_\vh(1) + \phi_\vh(-1)] = \bE_\vh[\phi_\vh(1)],
% \end{align*}
% and so, $\cL_\mu(\mW) = \bE_{\vh\sim \mu,\vz \sim \cN(\0, \bSigma)}[(\tanh((\vh^T+\vz^T)\mW\vh)-1)^2]$. Notice that although the minimizer $\mW^* = \bSigma^{-1}$ of $\cL$ is independent of the distribution $\mu$ of $\vh$, the minimum value $\cL_\mu(\bSigma^{-1})$ depends on $\mu$. Noting that $1-\tanh(z) = 1 - \frac{1-e^{-2z}}{1+e^{-2z}} = \frac{2e^{-2z}}{1+e^{-2z}} = \frac{2}{1+e^{2z}}$, we can write $\cL_\mu(\mW; \bSigma) = \bE_{\vh\sim \mu}[\psi_\vh(\mW; \bSigma)]$, where
% \begin{align*}
%     \psi_\vh(\mW; \bSigma) \triangleq \bE_{\vz\sim\cN(\0, \bSigma)}[(1-\tanh((\vh^T+\vz^T)\mW\vh))^2]= 4\bE_{\vz\sim \cN(\0,\bSigma)}\Big[\frac{1}{(1+\exp(2(\vh^T+\vz^T)\mW\vh))^2}\Big].
% \end{align*}
% The result from the previous section is that for any $\0 \prec \bSigma \in\bR^{d\times d}, \vh\in \bR^d$, we have $\psi_\vh(\mW; \bSigma) \ge \psi_\vh(\bSigma^{-1}; \bSigma)$ for all $\mW \in \bR^{d\times d}$.

% \subsubsection{Detour to verify the above claim}
% Let $d = 1, \bSigma = \sigma^2 > 0, \mW = \omega$. Then, we have that $\psi_h(\omega;\sigma^2) \ge \psi_h(\sigma^{-2}; \sigma^2)$ for any $\omega \in \bR$.
% \begin{align*}
%     \psi_h(\omega; \sigma^2) &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{\exp(-z^2/2\sigma^2)}{(1+\exp(2\omega h(h+z)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp(z^2/\sigma^2)+\exp(z^2/\sigma^2+2\omega h(h+z)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp((z/\sigma)^2)+\exp((z/\sigma)^2+2(\omega\sigma h)(z/\sigma) + \omega^2\sigma^2h^2+(2\omega h^2-\omega^2\sigma^2 h^2)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp((z/\sigma)^2)+\exp(h^2(2\omega-\omega^2\sigma^2))\exp((z/\sigma + \omega \sigma h)^2))^2} dz .
% \end{align*}
% The intuition is that we wish to maximize $\kappa(\omega;\sigma^2) \triangleq 2\omega-\omega^2\sigma^2$ in the denominator in order to minimize the above function, which happens at $\omega^* = \sigma^{-2}$.

% Clearly $\kappa$ is concave in $\omega$. Does this imply that $\psi_h(\omega; \sigma^2)$ is convex in $\omega$?

% \subsection{Effect of the covariance}
% If $\vh \sim \cN(\0, \bSigma)$, and $\vh$ is known (or in the regime of obtaining a good estimate of it, for example large $N$), then the optimal estimate of $y$ from $\vx = \vh y + \vz$, $\vz \sim \cN (\0, \sigma^2\mI_d)$ is $\hat{y} = \frac{\vh^T \vx}{\norm{\vh}_2^2 + \sigma^2}$



% We aim to show that when $N$ is large $\mW = \alpha \mI_d$ for some $\alpha \ge 0$ large.





==> AISTATS-2025/contents-AISTATS/wireless-communication-model.tex <==

\section{Wireless Communication System Model}
\label{wireless_communication_problem}

In this section, we specialize the estimation problem stated in Section \ref{in_context_estimation} to the wireless communication problems of interest.
Consider a wireless channel with a single transmit antenna and $d$ receive antennae (see Fig. \ref{fig:TranEstimator}). Let $s_t \in \cX = \{x_I+ \sqrt{-1} \ x_Q  \mid x_I, x_Q\in\{\pm 1\}\}$ be the $t$th transmitted symbol.
The transmit sequence $\{s_t\}$ is an i.i.d sequence of symbols drawn from $\cX$ with uniform probability.

Let $\vy_t \in \bC^d$ be the received symbol vector, where $y^j_t$ denotes the received symbol at the $j$th antenna at time $t$. 
Let $\vh_t(\theta) \in\bC^d$ be the wireless channel coefficient between the transmitter and the $j$th receiver antenna, and let $\vz_t$ be the additive noise at the receiver, at time $t$. 
Then, we can write the input-output relation as
\begin{equation}
\label{eq:io_relation}
    \vy_t = \vh_t(\theta) s_t + \vz_t, \quad t\in[\ell].
\end{equation}



%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure below %%%%%%%%%%%%%
\begin{figure}[ht]
\centering
\input{figures/TranEstimator}
\caption{Notional diagram of a typical single-input multiple-output (SIMO) wireless channel combined with a transformer-based receiver}
\label{fig:TranEstimator}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure above %%%%%%%%%%%%%

For some $\sigma^2 > 0$, the sequence $\{\vz_t\}$ are independent and identically distributed (i.i.d.) Gaussian random vectors, with $\vz_{t, I},\vz_{t,Q}\sim \mathcal{N}(\mathbf{0}, \sigma^2 \mI_{d})$ for each $t\in[\ell]$. The ratio $1/\sigma^2$ is called the signal-to-noise-ratio (SNR).




Next, we describe the latent context space $\Theta$, and the conditional distributions for the channel, i.e., $P_{h\mid \theta}$ for $\theta\in\Theta$. The channel parameter process $\{\vh_t(\theta)\}$ in the wireless communications typically depends on two aspects, discussed in the following subsections.


\subsection{Type of Scattering}

In wireless communication, signals transmitted from the transmitter antenna reach the receiver antenna from multiple directions after being scattered by the obstacles in the environment. In this situation, the channel parameter depends on the configuration of the environment and the positioning and influence of the obstacles. If there are few or no obstacles, there is a direct path called the line-of-sight (LoS) path between the transmitter and the receiver, and in this case, the received signal can be modeled by a single ray of signal reaching the antenna. Thus, the effective channel parameter depends on the angle of arrival of this LoS component of the signal. On the other hand, if there are significantly many scatterers in the environment, as in an urban environment, there is a large number of reflected rays reaching the receiver at the same time. This scenario is (aptly) called the rich-scattering environment, and the channel parameter in this case can be approximated as a Gaussian random variable. 

Each of the above cases gives rise to a different distribution on the channel, and hence, we model the type of scattering of the signal as the latent context $\theta$. More formally, let $\Theta=\{0, 1\}$ denote the latent context space where $\theta = 0$ corresponds to the LoS model, and $\theta=1$ corresponds to the rich scattering model. In this case, we first generate $\vh_1(\theta)$ and assume that it remains constant for the period of interest, i.e., $\vh_t(\theta) = \vh_1(\theta)$ for all $t\in[\ell]$. This corresponds to the environment being stationary, i.e., the signal paths do not change over time in the period of interest.

    When $\theta=0$, $h_1^j(0) = \exp(-(\sqrt{-1})2\pi (s/\lambda)(j-1)\cos(\alpha)) \triangleq \phi_j(\alpha)$, where $j\in[d]$. 
    
    Here, $\alpha \sim {\rm Unif}[0, \pi)$ is the angle of arrival of the one ray (\cite{goldsmith_2005}), $s$ is the spacing between the antennae, $\lambda$ is the wavelength of the signal used for transmission.

    When $\theta=1$, the channel parameter is modeled by $\vh_{1, I}(1),\vh_{1, Q}(1) \sim \mathcal{N}(0, \frac{1}{2}\mI_d)$, with $\vh_{1, I}(1), \vh_{1, Q}(1)$ are drawn independently. We call the above case as scenario C1.

\subsection{Mobility}

Assume that the transmitter is fixed and the receiver is moving towards the transmitter with some velocity $v$ m/s. This situation naturally arises in the wireless communication application. Considering a rich-scattering environment, the properties of the channel parameter, and the correlation of the parameter process depends on the velocity: more the velocity, less the correlation. Therefore, having a estimate of the velocity in such environments and the correlation structure would greatly improve the performance of the estimator at the receiver. However, in practice, this can be difficult to obtain online. Hence, we model velocity to parameterize the latent context $\theta$. 

More specifically, we consider a latent space $\Theta = [M]$  representing the $M$ possible velocities with $v_\theta$ being the mobile velocity when the latent variable is $\theta$. Let $\{h^j_t(\theta)\}_t$ denote the channel parameter process at the $j$th antenna. Note that this process is a time-varying process with unlike in the last scenario, where the process that remains constant across the time. Across the antennae $j\in[d]$, we assume that the processes $\{h^j_t(\theta)\}_t$ are  i.i.d. zero-mean, wide-sense stationary Gaussian random processes (Section 15.5, \cite{Kay97}). The correlation function $R_\theta(m) = \bE[h_{t, I}^1(\theta) h^1_{m+t, I}(\theta)]$ for any $t\in\bN$ is determined by the latent context $\theta$. We use the well-known Clarke's model (Section 3.2.1, \cite{goldsmith_2005})and set $R_\theta(m) = J_0(\frac{2\pi T_s m v_\theta}{\lambda})$. Here, $T_s$ is the symbol duration, $\lambda$ is the wavelength of the signal, $v_\theta$ is the relative velocity between the transmitter and the receiver, $J_0$ denotes the Bessel function of the first kind of order $0$. 
We call the above scenario as scenario C2.


In both the scenarios C1 and C2, the latent parameter $\theta$ is drawn uniformly at random from $\Theta$. 


In wireless communications, a set of known symbols called pilots are transmitted as part of the transmitted symbols. 
These symbols are used to estimate the channel parameter process and then the estimate is typically used to perform symbol estimation. 
There is a natural way in which these pilots can be used as in-context examples. 
In the language of Section \ref{in_context_estimation}, the set $S_k$ contains the pilots symbols $(s_t, t\in[k])$ until time $k$
and the corresponding received symbols $(\vy_t, t\in[k])$. 
The pilots do not communicate any information and hence, it is important to keep the number of pilots small. 
Thus, machine learning model based estimators need to be information-efficient and make maximal use of the information in $S_k$.


==> contents/abstract-neurips.tex <==
\begin{abstract}
 Pre-trained transformers exhibit the capability of adapting to new tasks through in-context learning (ICL), where they efficiently utilize a limited set of prompts without explicit model optimization.
 The canonical communication problem of estimating transmitted symbols from received observations can be modelled as an in-context learning problem: Received observations are essentially a noisy function of transmitted symbols, and this function can be represented by an unknown parameter whose statistics depend on an (also unknown) latent context. This problem, which we term in-context estimation (ICE), has significantly greater complexity than the extensively studied linear regression problem.
 The optimal solution to the ICE problem is a non-linear function of the underlying context. In this paper, we prove that, for a subclass of such problems, a single layer softmax attention transformer (SAT) computes the optimal solution of the above estimation problem in the limit of large prompt length. We also prove that the optimal configuration of such transformer is indeed the minimizer of the corresponding training loss. Further, we empirically demonstrate the proficiency of multi-layer transformers in efficiently solving broader in-context estimation problems. Through extensive simulations, we show that solving ICE problems using transformers significantly outperforms standard approaches. Moreover, just with a few context examples, it achieves the same performance as an estimator with perfect knowledge of the latent context. 
\end{abstract}



% Pre-trained transformers can perform in-context learning, where they adapt to a new task using only a small number of prompts without any explicit model optimization. 

% Inspired by this attribute, we propose a novel approach, called in-context estimation, for the canonical communication problem of estimating transmitted symbols from received symbols.


% A communication channel is essentially a noisy function that maps transmitted symbols to received symbols, and this function can be represented by an unknown parameter whose statistics depend on an (also unknown) latent context. 
% Conventional approaches typically do not fully exploit hierarchical model with the latent context. Instead, they often use mismatched priors to form a linear minimum mean-squared error estimate of the channel parameter,
% which is then used to estimate successive, unknown transmitted symbols. We make the basic connection that transformers show excellent contextual sequence completion with a few prompts, and so they should be able to implicitly determine the latent context from pilot symbols to perform end-to-end in-context estimation of transmitted symbols. Furthermore, the transformer should use information efficiently, i.e., it should utilize any pilots received to attain the best possible symbol estimates. Through extensive simulations, we show that in-context estimation not only significantly outperforms standard approaches, but also achieves the same performance as an estimator with perfect knowledge of the latent context within a few context examples. Thus, we make a strong case that transformers are efficient in-context estimators in the communication setting.


   %  Pre-trained transformers can perform in-context learning, where they adapt to a new task using only a small number of prompts without any explicit model optimization.  

   % The canonical communication problem of estimating transmitted symbols from received symbols can be modelled as an in-context learning problem: The received symbols are essentially a noisy function of transmitted symbols, and this function can be represented by an unknown parameter whose statistics depend on an (also unknown) latent context. 

   % This problem is significantly more challenging than the well-studied linear regression problem, as the optimal solution of this problem is a non-linear function of the underlying context.

   %  In this paper, we demonstrate the ability of transformers for this class of problems, referred to as In-context Estimation (ICE).

  


% This problem poses a notably greater complexity compared to the extensively studied linear regression problem, given that its optimal resolution entails a non-linear function of the underlying context.

% This paper showcases the proficiency of transformers in addressing this category of problems, which we term In-context Estimation (ICE).

    
    
    % for the canonical communication problem of estimating transmitted symbols 
    
    % A communication channel is essentially a noisy function that maps transmitted symbols to received symbols, and this function can be represented by an unknown parameter whose statistics depend on an (also unknown) latent context. 

    
    % Conventional approaches typically do not fully exploit hierarchical model with the latent context. 
    
    % Instead, they often use mismatched priors to form a linear minimum mean-squared error estimate of the channel parameter, which is then used to estimate successive, unknown transmitted symbols.

    
    % We make the basic connection that transformers show excellent contextual sequence completion with a few prompts, and so they should be able to implicitly determine the latent context from pilot symbols to perform end-to-end in-context estimation of transmitted symbols. Furthermore, the transformer should use information efficiently, i.e., it should utilize any pilots received to attain the best possible symbol estimates. Through extensive simulations, we show that in-context estimation not only significantly outperforms standard approaches, but also achieves the same performance as an estimator with perfect knowledge of the latent context within a few context examples. Thus, we make a strong case that transformers are efficient in-context estimators in the communication setting. 

==> contents/additional-related-work.tex <==

\section{Related Work} 
The in-context learning abilities of the transformer were first showcased by \citet{LanguageModelsAreFewShotLearners} where GPT-3, a transformer-based large language model, was shown to perform well on novel, unseen tasks in a few-shot or zero-shot manner. The authors of \cite{xie2022an} used synthetic data to show that in-context learning can be interpreted as Bayesian inference, wherein a model first attempts to infer the task and then uses this prediction to carry out the task.

In \cite{garg2023transformers}, authors look at in-context learning as a problem of learning to perform linear regression by being trained on sequence data, rather than learning in the natural language setting. The authors of \cite{panwar2024incontext} build on this work and provide mathematical theory to describe how this can be interpreted as the model performing Bayesian inference by estimating a posterior distribution. These two works are closely related to our work.

Other work has gone further in explaining the mechanisms by which transformers are able to perform in-context learning. Some authors have explored the behavior of simplified transformer models on synthetic linear regression problems, as compared to the globally optimal solutions for these problems\cite{mahankali2023step,zhang2024trained}.
In \cite{whatlearningalgorithm}, it is shown by construction that transformers can learn to fit a linear model at inference time given a context. This tells us that, at least in theory, transformers can learn to literally perform regression and related computations given some data. A related line of work explores the manner by which transformer models carry out these optimization procedures and shows that transformer models can perform nontrivial gradient-based optimization procedures at inference time\cite{von2023transformers,ahn2024transformers}. 
In \cite{EmergentICL}, the authors test how properties of training data impact in-context learning behaviors. 
The authors of \cite{min2022rethinking} similarly study how the properties of the context itself impact in-context learning performance. 

In summary, many different research directions have provided ways to interpret and understand in-context learning and the mechanisms by which transformer models do it. In our work, we primarily use the Bayesian perspective to view this ability and to understand how we can apply it to the wireless communication domain.

% \subsection{Machine Learning for Wireless Communication}

The problem of symbol estimation in the presence of an unknown channel is a canonical problem in wireless communication and there is a large body of literature that considers model-driven traditional signal processing approaches. 
When the prior distribution for the channel follows a hierarchical model with latent contexts such as what we study in this paper, optimal model-based estimators become computationally infeasible. 
While approximations to the optimal estimators have been studied with restricted priors, the structure and performance of such estimators are highly dependent on the priors.

Recently, there has been significant interest in using machine learning methods such as variational inference \cite{ChannelEstimationUsingVAE}, \cite{UnsupervisedEqualizationUsingVAEs} and deep neural network models such as fully connected neural networks \cite{DeepLearningAidedChannelEstimation}, convolutional neural networks \cite{LearningMMSEChannelEstimator}, and recurrent neural networks \cite{RNNforChannelEstimation} 
for channel estimation and for symbol estimation \cite{aoudia2021end}. The authors of \cite{faycal} design an  end-to-end wireless communication system design using learning-based approach.
The work of \cite{neumann} provides a principled way of designing channel estimators in the setting of wireless communication, by training CNN-based neural network to efficiently estimate the channel parameters when it follows a hierarchical prior. The authors of \cite{UnsupervisedLinearAndNonLinearChannelEqAndDecoding} used variational autoencoders (VAEs) and unsupervised learning to implicitly learn and decode symbols in a wireless channel. In \cite{burshtein2023semi}, the authors use VAEs in a semi-supervised setting to operate over non-linear channels. The approach in \cite{deepLearningForTimeVaryingMIMOChannels} uses a long short-term memory (LSTM) based channel parameter estimator for a time-varying channel. They are interested in learning the spatial correlation structure of the channel coefficients across the receiver antennae.
 
 The main distinction of our work from the previous works is that we make the connection between the in-context learning capabilities of the transformer and the symbol estimation problem in wireless communication. We show how the problem fits naturally in the setting, and provide empirical evidence that transformers achieve near-optimal performance. A comparative study of the performance of the transformers and other machine learning models is left for the future work.

% \subsection{Transformers and In-Context Learning}
% Transformer architectures \cite{NIPS2017_3f5ee243} have become a popular model across various problems due to the effectiveness of multi-head self-attention units on a wide variety of natural language tasks. \citet{LanguageModelsAreFewShotLearners} demonstrated that GPT-3, a transformer-based large language model, performs well on novel, unseen tasks in few-shot or zero-shot settings, known as in-context learning. \citet{xie2022an} used synthetic data to show that in-context learning can be interpreted as Bayesian inference, where a model first infers the task and then uses this prediction to execute the task.

% In \cite{garg2023transformers}, authors explore in-context learning from a different perspective by training models on sequence data to perform least-squares estimation for linear regression. Authors of \cite{ahuja2023incontext} extend this by providing a mathematical theory that interprets the model's performance as Bayesian inference by estimating a posterior distribution. These papers \cite{garg2023transformers} and \cite{ahuja2023incontext} are closely related to our work

% Other works have further explored the mechanisms behind transformers' in-context learning. Simplified transformer models on synthetic linear regression problems have been compared to globally optimal solutions~\cite{mahankali2023step,Zhang2023TrainedTL}. \cite{whatlearningalgorithm} demonstrated that transformers could learn to fit a linear model at inference time given a context, indicating that transformers can theoretically perform regression and related computations with given data. Moreover, \cite{von2023transformers,ahn2024transformers} showed that transformer models could perform nontrivial gradient-based optimization procedures at inference time. \cite{EmergentICL} tested how training data properties impact in-context learning behaviors, while \cite{min2022rethinking} studied how the context's properties affect in-context learning performance.

% In summary, various research directions have provided insights into in-context learning and the mechanisms by which transformer models achieve it. Our work primarily adopts a Bayesian perspective to understand and apply this ability to the wireless communication domain.

% \subsection{Machine Learning for Wireless Communication}
% Symbol estimation in the presence of an unknown channel is a canonical problem in wireless communication, extensively studied using model-driven traditional signal processing approaches. When the channel's prior distribution follows a hierarchical model with latent contexts, optimal model-based estimators become computationally infeasible. While approximations to optimal estimators have been studied with restricted priors, their structure and performance heavily depend on the priors.

% Recently, there has been significant interest in using machine learning methods for channel estimation, such as variational inference~\cite{ChannelEstimationUsingVAE,UnsupervisedEqualizationUsingVAEs} and deep neural network models like fully connected neural networks~\cite{DeepLearningAidedChannelEstimation}, convolutional neural networks~\cite{LearningMMSEChannelEstimator}, and recurrent neural networks~\cite{RNNforChannelEstimation}. \cite{aoudia2021end} designed an end-to-end wireless communication system using a learning-based approach. \cite{faycal} proposed a principled method for designing channel estimators in wireless communication by training CNN-based neural networks to estimate channel parameters efficiently under hierarchical priors. \cite{UnsupervisedLinearAndNonLinearChannelEqAndDecoding} used variational autoencoders (VAEs) and unsupervised learning to implicitly learn and decode symbols in a wireless channel, while \cite{SemisupervisedVAEForNonLinearChannels} employed VAEs in a semi-supervised setting for non-linear channels. \cite{deepLearningForTimeVaryingMIMOChannels} utilized an LSTM-based channel parameter estimator for time-varying channels, focusing on learning the spatial correlation structure of the channel coefficients across receiver antennas.

% Our work distinguishes itself by connecting the in-context learning capabilities of transformers to the symbol estimation problem in wireless communication. We show how the problem fits naturally in this setting and provide empirical evidence that transformers achieve near-optimal performance. A comparative study of the performance of transformers and other machine learning models is left for future work.

% % \section{Related Work}

% % \subsection{Transformers and In-Context Learning}

% % Transformer architectures have gained popularity for their strong performance across various problems, particularly due to the effectiveness of multi-head self-attention units in natural language tasks ~\cite{NIPS2017_3f5ee243}. Notably, in \cite{LanguageModelsAreFewShotLearners} GPT-3 has shown the ability to perform well on novel tasks in a few-shot or zero-shot manner, known as in-context learning. This process has been interpreted as Bayesian inference, where the model first infers the task and then uses this prediction to perform the task.

% % Our approach closely relates to studies by \cite{garg2023transformers}  and \cite{ahuja2023incontext}. \cite{garg2023transformers} explored in-context learning through the lens of least-squares estimation for linear regression, using sequence data for training. \cite{ahuja2023incontext} extended this by providing a mathematical framework to describe in-context learning as Bayesian inference. Additional research has further examined how transformers perform in-context learning, including simplified models on synthetic linear regression problems and gradient-based optimization procedures at inference time. Studies have also looked at the impact of training data properties and context properties on in-context learning.

% % Overall, various research directions have enhanced our understanding of in-context learning and the mechanisms by which transformers achieve it. Our work primarily adopts a Bayesian perspective to apply this capability to the domain of wireless communication.

% % \subsection{Machine Learning for Wireless Communication}

% % Symbol estimation under channel uncertainty is a well-studied problem in wireless communication, traditionally approached with model-driven signal processing techniques.
% % Optimal model-based estimators often become computationally infeasible when the channel exhibit intricate behavior, e.g., when its prior distribution follows a hierarchical model with latent contexts.
% % Recent interest has shifted towards machine learning methods for channel and symbol estimation. These include variational inference, fully connected neural networks, convolutional neural networks, recurrent neural networks, and end-to-end system designs using learning-based approaches.
% % For example, \cite{neumann} trained CNNs for channel parameter estimation under hierarchical priors, and variational autoencoders have been used for unsupervised and semi-supervised learning in non-linear channels. LSTM-based estimators have also been employed for time-varying channels to learn spatial correlation structures.

% % Our work distinguishes itself by connecting the in-context learning capabilities of transformers with the symbol estimation problem in wireless communication, demonstrating near-optimal performance.
% % Future work will include a comparative study of transformers against other machine learning models.

==> contents/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} %, \answerNo{}, or \answerNA{}.\answerYes{}
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Assumptions have been clearly stated, and all proofs and baselines are available in the appendix \ref{sec:appendix-finite-estimation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training details have been provided in \ref{parameters}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training details have been provided in \ref{parameters}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:  \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Typically Mean squared error plots aren't computed with error bars in wireless communication works.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Training details have been provided in \ref{parameters}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the introduction, we allude to the fact that our results, which show the estimation abilities of transformers could make them a potential building block of future wireless systems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper cites \citet{radford2019language} as we use the GPT2 model, and \citet{panwar2024incontext} as we use parts of their codebase.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The details of our contributions have been detailed in the readme file.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> contents/conclusion.tex <==
\section{Conclusion}

In conclusion, our research demonstrates that pre-trained transformers can effectively adapt to new tasks through in-context learning (ICL), leveraging a limited set of prompts without explicit model optimization. We framed the canonical communication problem of estimating transmitted symbols from received observations as an in-context learning problem, which we termed in-context estimation (ICE). 

% This problem involves a noisy function of transmitted symbols represented by an unknown parameter whose statistics depend on an unknown latent context, presenting a complexity significantly greater than the well-studied linear regression problem due to its non-linear optimal solution.

Our findings show that, for a subclass of ICE problems, a single-layer softmax attention transformer (SAT) can compute the optimal solution in the limit of large prompt lengths. We provided proof that the optimal configuration of such a transformer is indeed the minimizer of the corresponding training loss. Additionally, our empirical results highlight the efficiency of multi-layer transformers in addressing broader ICE problems.
Simulations confirm that transformers not only outperform standard approaches but also match the performance of an estimator with perfect knowledge of the latent context using only a few context examples. These results underscore the potential of transformers in efficiently solving complex estimation problems in communication systems.

% Across the various tasks, parameters, and regimes studied, transformer models are able to infer the latent context from a few samples and then use this information to make an accurate estimation of $\vx_{k+1}$. We use genie-aided context-aware estimators to find lower bounds on the performance of any such model. These estimators are given exact, noiseless information about the context, which is not available to the transformer model. Even without such extra information, the transformer models we trained are able to approach and reach the performance of the context-aware methods. This finding demonstrates that the ability of transformers to learn in-context from prompts enables these models to perform well on wireless communication problems.

==> contents/detection-loss.tex <==
\section{Softmax attention with cross-entropy loss}

Let $\cS$ be the signal set be the input symbols, and let $S \triangleq \abs{\cS}$. Let $y_n = H s_{x_n} + z_n$, where $x_n \sim [S]$ and $z_n \sim \cN(0, \Sigma)$. Let $(y_n, e_{x_n}, n\in[N])$, and let $y_{q}$ be the query received symbol. Now, the attention applied to the sequence of symbols is
\begin{align*}
    p^{\rm tr}(y_q, \{y_n, & x_n\}_{n\in[N]}; \mW) = \frac{\sum_{n\in[N]}e_{x_n} \exp(y_q^T \mW y_n)}{\sum_{n\in[N]} \exp(y_q^T \mW y_t)} \\
    &= \frac{\sum_{i\in[S]} e_i \sum_{n\in \cT_i}\exp(y_q^T \mW y_n) }{\sum_{i\in[S]}  \sum_{n\in \cT_i} \exp(y_q^T \mW y_n)},
\end{align*}
where the sets $\cT_i \triangleq \{n\in[N]: x_t = i\}$, and $N_i \triangleq \abs{\cT_i}$, with $[N] = \sqcup_{i\in[S]} \cT_i$ and $N = \sum_{i} N_i$. Thus, $p^{\rm tr}_i(y_q, \{y_t, x_t\}_{n\in[N]}; \mW) = \frac{ \sum_{n\in \cT_i}\exp(y_q^T \mW y_n) }{\sum_{i\in[S]}  \sum_{n\in \cT_i} \exp(y_q^T \mW y_n)}$, which is a simple-soft nearest neighbour estimator. The population loss is given by
\begin{align*}
    \cL_T(\mW) \triangleq \bE_{X_0^{T-1}, Y_0^{T-1}, X_q, Y_q}\left[- \sum_{i\in[S]} p_i(Y_q, Y_0^{T-1}, X_0^{T-1}) \log p_i^{\rm tr}(Y_q, Y_0^{T-1}, X_0^{T-1}; \mW) \right].
\end{align*}


\subsection{Asymptotic analysis of the transformer estimator}

In this section, we analyse the transformer detector and loss when $T \to \infty$. Clearly, 
\begin{align*}
     \lim_{T\to \infty} p^{\rm tr}(y_q, \{y_t, x_t\}_{n\in[N]}; \mW) = \frac{\sum_{i\in[S]} e_{i} \exp(y_q^T \mW H s_{i})}{\sum_{i\in[S]} \exp(y_q^T \mW H s_{i})} \triangleq \hat{p}(y_q; \mW).
\end{align*}

If $H^T H = I$ (the columns for $H$ are orthonormal), and $s^T s = \gamma$ for all $s\in \cS$ (constant power signal set), then $\hat{p}_i(y_q; \Sigma^{-1}) = \bP[X_q = i \mid Y_q=y_q]$ is the true posterior.

Consider the cross-entropy loss at infinite prompt length during training:
\begin{align*}
    \cL(\mW) &\triangleq -\bE_{X_q, Y_q}\left[\log \hat{p}_{X_q}(Y_q; \mW)\right] = -\bE_{X_q, Y_q}\left[ \bE [\log \hat{p}_{X_q}(Y_q; \mW) \mid Y_q]\right] \\
    &= -\bE_{X_q, Y_q} \left[ \bE_{X_q \sim \hat{p}(Y_q; \Sigma^{-1})}[\log \hat{p}_{X_q}(Y_q; \mW)] \right] = \bE_{X_q, y_q} [D_{\rm KL}[\hat{p}(Y_q; \Sigma^{-1}) \lVert \hat{p}(Y_q; \mW)]] + \bH[P_{X,Y}].
\end{align*}

\begin{lemma}
\label{lem:strict-convexity-of-cross-entropy}
    Let $\ell_q(z) \triangleq H(q, p(z)) = -\sum_{i\in[S]} q_i \log p_i(z)$ for $z \in \bR^{S}$, where $p_i(z) \triangleq {\rm softmax}_i(z) = \frac{e^{z_i}}{\sum_{j\in [S]}e^{z_j}}$, for some $q \in \Delta^S$, i.e., $q_i \ge 0, n\in[S]$ and $\sum_{i\in[S]} q_i = 1$. The function $\ell_q$ is strictly convex for all $q\in\Delta^S$. Let $h: V \to \bR^S$ be a linear map from a vector space $V$ to $\bR^S$. The function $g_{q,h}: V \to \bR$ defined as $g_{q, h}(\theta) = \ell_q(h(\theta))$ is strictly convex in $\theta$.
\end{lemma}
\emph{Proof}. We can directly compute the components of the gradient as
\begin{align*}
     [\nabla_z \ell_q(z)]_j =  -\sum_{i\in[S]} q_i \left(\frac{\partial}{\partial z_j}  (\log p_i(z)) \right) = -\sum_{i\in[S]} q_i \left(\frac{1}{p_i(z)} \frac{\partial p_i(z)}{\partial z_j} \right) \stackrel{(1)}{=} -\sum_{i\in[S]} q_i (\delta_{ij}-p_j(z)) = p_j(z)-q_j.
\end{align*}
where $(1)$ follows from the derivatives of softmax function given by
\begin{align*}
    \frac{\partial p_i(z)}{\partial z_j} = p_i(z)(\delta_{ij}-p_{j}(z)),
\end{align*}
whence $\nabla_z \ell_q(z) = p(z)-q$. Now, for any $z^1, z^2 \in \bR^S$, for any $i\in[S]$
\begin{align*}
    \log \left(\frac{p_i(z^1)}{p_i(z^2)}\right) = (z^1_i-z^2_i) + \log \left(\frac{\sum_{j\in[S] } e^{z^2_j}}{\sum_{j\in[S]} e^{z^1_j}}\right) \triangleq (z^1_i-z^2_i) + c(z^2, z^1),
\end{align*}
where $c(z^2, z^1)$ does not depend on the index $i$. Since 
\begin{align*}
    \ell_q(z^2)-\ell_q(z^1) - \langle \nabla_z \ell_q(z^1), z^2-z^1 \rangle 
    &= \sum_{i\in[S]} q_i \log \left(\frac{p_i(z^1)}{p_i(z^2)}\right) + \sum_{i\in[S]} (p_i(z^1) - q_i)(z^1_i-z^2_i) \\
    &= \sum_{i\in[S]} q_i \log \left(\frac{p_i(z^1)}{p_i(z^2)}\right) + \sum_{i\in[S]} (p_i(z^1) - q_i) \left(\log \left(\frac{p_i(z^1)}{p_i(z^2)}\right) - c(z^2, z^1) \right) \\
    &= \sum_{i\in[q]} p_i(z^1) \log \left( \frac{p_i(z^1)}{p_i(z^2)}\right) -c(z^2, z^1) \left( \sum_{i\in[s]} p_i(z^1) - \sum_{i\in[S]} q_i\right) = D_{\rm KL}[p(z^1) \lVert p(z^2)] > 0,
\end{align*}
if $z^1 \neq z^2$, the function $\ell_q$ is strictly convex. For any $\lambda \in(0,1)$, for any $\theta_1, \neq\theta_2 \in V$, we have
\begin{align*}
    g_{q,h}(\lambda  \theta_1 + (1-\lambda)\theta_2) &= \ell_q(h(\lambda  \theta_1 + (1-\lambda)\theta_2)) = \ell_q(\lambda h(\theta_1) + (1-\lambda) h(\theta_2)) \\
    &< \lambda \ell_q(h(\theta_1)) + (1-\lambda) \ell_q(h(\theta_2)) = \lambda g_{q,h}(\theta_1) + (1-\lambda) g_{q,h}(\theta_2),
\end{align*}
whence $g_{q,h}$ is strictly convex.

\begin{theorem}
\label{thm:strict-convexity-of-loss}
The loss function $\cL: \bR^{d\times d} \to \bR$ is strictly convex in the attention weights, and $\mW^* = \Sigma^{-1}$ is the global minimizer of $\cL$.
\end{theorem}
\emph{Proof}. Let $V = \bR^{d\times d}$. For a fixed $Y_q(\omega) = y_q$, let $h_i(\mW; y_q) = y_q^T \mW H s_i$ for $i\in[S]$ and $q(y_q) = \hat{p}(y_q; \Sigma^{-1}) \in \Delta^S$. Therefore, $g_{h, q}(\mW; y_q)$ is strictly convex from Lemma \ref{lem:strict-convexity-of-cross-entropy}, whence $\cL(\mW) = \bE_{X_q, Y_q}[g_{h, q}(\mW; Y_q)]$ is strictly convex in $\mW$. Minimizer follows from the KL-characterization of $\cL$.



\subsection{Non asymptotic analysis of the estimator and loss function}

Let $(V, \norm{\cdot})$ be a normed linear space, and let $\mu: V \to \bR^S, \sigma: V \to \bR$ be linear maps. Let $r: V \to \Delta^S$ be a stochastic function given by
\begin{align*}
    r^T_i(\theta, z) = \frac{ T_i e^{\mu_i(\theta)} \left(\frac{1}{T_i}\sum_{n\in [T_i] } e^{\sigma(\theta)z_t}\right)}{\sum_{j\in [S]} T_j e^{\mu_j(\theta)} \left(\frac{1}{T_j}\sum_{s\in[T_j]}e^{\sigma(\theta)z_s} \right)},
\end{align*}
where $z \sim \cN(\0,\mI_T)$. Assuming a prior $\rho \in \Delta^S$, we have $T_i/T \to \rho_i$ a.s., and so almost surely, we have
\begin{align*}
    r_i(\theta) = \lim_{T\to \infty} r^T_i(\theta, z) = \frac{e^{\mu_i(\theta) + \log \rho_i}}{\sum_{j\in[S]}e^{\mu_j(\theta) + \log \rho_j}} = {\rm softmax}_i(\mu(\theta)+\rho).
\end{align*}
We showed that $\cL(\theta) = -\sum_{i\in[S]} q_i \log r_i(\theta)$ is convex in $\theta$.

For $i\in[S]$, consider:
\begin{align*}
    \ell^T_i(\theta) \triangleq -\bE_{z}[\log r^T_i(\theta, z)]
\end{align*}

Note that $\cL_T(\theta) = \sum_{i\in[S]} q_i \ell^T_i(\theta)$.


==> contents/in-context-estimation.tex <==
\section{In-Context Estimation}
\label{sec:in-context-estimation}
In this section, we define the problem of in-context estimation, and we discuss the complexities associated with solving it.
\begin{definition}
\label{def:ice}
{\bf (In-Context Estimation)} Let $\{\vx_t\}_{t=1}^{n+1} \stackrel{\rm iid}{\sim} \bP_x$ be the input symbols and $ \{\vz_t\}_{t=1}^{n+1} \stackrel{\rm iid}{\sim}  \bP_z$ be the noise samples. Let $\{\mH_t(\theta)\}_{t=1}^{n+1} \sim \bP_{h \mid \theta}$ be a random process determined by a latent parameter $\theta \sim \bP_\Theta$. For $t\in[n+1]$, $\vy_{t} = \vg(\vx_t, \mH_t(\theta)) + \vz_t$. Let $\cP^n_\theta \triangleq \{(\vy_t, \vx_t), t\in[n]\}$ to be the set of examples in the prompt until time $n$. The problem of in-context estimation (ICE) involves estimating $\vx_{n+1}$ from $\vy_{n+1}, \cP_{\theta}^n$ such that the mean squared error (MSE) $\bE_{\theta \sim \bP_\Theta, \{\mH(\theta)\} \sim \bP_{h\mid \theta}, \vz\sim \bP_z, \vx\sim \bP_x}[\norm{\hat{\vx}_{n+1}( \cP_\theta^n, \vy_{n+1})-\vx_{n+1}}_2^2]$ is minimized.
\end{definition}

For the above problem, consider the following estimator. Given the past $n$ examples $\cP_\theta^n$ from the context $\theta\in \Theta$ and the current observation $\vy_{n+1}$, the context unaware (CU) minimum mean squared error estimate (MMSE) of $\vx_{n+1}$ is known to be the conditional mean estimate (CME)
\begin{equation}
\label{eq:context_agnostic_estimator}
    \hat{\vx}_{n+1}^{\rm CU}(\cP_\theta^n, \vy_{n+1}) = \bE[ \vx_{n+1} = \vx \mid \cP_\theta^n, \vy_{n+1}].
\end{equation}

% In addition, if the estimator knows the latent context parameter $\theta$ apriori, then the context aware (CA) optimal estimator is given by
% \begin{equation}
% \label{eq:in_context_estimator}
%     \hat{\vx}_{n+1}^{\rm CA}(\cP_\theta^n, \vy_{n+1};\theta) = \bE_{\vx \sim \bP_x}[ \vx_{n+1} = \vx \mid \cP_\theta^n, \vy_{n+1}, \theta],
% \end{equation}
% which we call the optimal context-aware estimator. It is known that the MSE achieved by an optimal context-aware estimator not worse than that of a context agnostic estimator given by Equation \ref{eq:context_agnostic_estimator}.

Having a closer look at the computation of the conditional expectation in \eqref{eq:context_agnostic_estimator}, we get
\begin{align*}
    &\hat{\vx}_{n+1}^{\rm CU}(\cP_\theta^n, \vy_{n+1}) = \bE[ \vx_{n+1} = \vx \mid \cP_\theta^n, \vy_{n+1}] = \sum_{\vx \in \cX} \vx \bP_x(\vx_{n+1} =  \vx \mid\cP_\theta^n, \vy_{n+1}) \\
    &\hspace{20pt} \propto \sum_{\vx\in \cX} \vx \bP_x(\vx) p(\cP_\theta^n, \vy_{n+1} \mid \vx) \\
    &\hspace{20pt} =\sum_{\vx\in \cX}\vx \bP_x(\vx) \int_{\theta' \in \Theta} p_\Theta(\theta')\int_{\mH_1, \dots, \mH_n, \mH_{n+1} \in \bR^{d_{\vy}\times d_{\vx}}} p_{h \mid \theta'}(\mH_1, \dots, \mH_n, \mH_{n+1}) \\
    &\hspace{50pt} p(\cP_\theta^n, \vy_{n+1} \mid \vx, \mH_{1}, \dots, \mH_n, \mH_{n+1})~ d\mH_1 \dots d\mH_{n+1}
\end{align*}
The above computation involves evaluating a multi-dimensional integral. In most practical problems of estimation, computation of \eqref{eq:context_agnostic_estimator} can be very difficult or even intractable. 

% We train a transformer and demonstrate its effectiveness in approximating Equation \ref{eq:context_agnostic_estimator}.

\begin{quote}
    Why can estimation problems be more challenging than the regression problems?
\end{quote}

To distinguish these two settings, consider the linear model $\vg: \bR^{d_\vx}\times \bR^{d_{\vy} \times d_{\vx}} \to \bR^{d_\vy}$ defined by $\vg(\vx, \mH) = \mH \vx$.
In the linear regression setting with the relation $\vy = \mH \vx$, the optimal estimate $\hat{\vy}$ obtained from observation $\vx$ and given $\mH$ is simply the linear transform $\hat{\vy} = \mH\vx = \vy$.
In other words, the optimal estimator is a linear function of the underlying context $\mH$; the optimal estimate has trivial (zero) error when the context $\mH$ is perfectly known.
On the other hand, the optimal estimate $\hat{\vx}$ of $\vx$ from the noisy $\vy = \mH \vx + \vz$ is not straightforward due to the presence of noise.
This difficulty arises due to the fact that the independent variable $\vx$ is to be estimated from a noisy dependent observation $\vy$ in the latter setting and, hence, the optimal estimate does not have a simple form.

Motivated by canonical estimation problems in wireless communication, we restrict our attention to the problem of estimating complex symbols under an unknown transformation embedded in Gaussian noise, and we show that it naturally fits into the above framework.
In this class of problems, the relationship between the input symbols and the observed symbols (in the complex domain) is captured by:
\begin{equation}
    \label{eq:complex-est-prob}
    \tilde{\vy}_t = \tilde{\vh}_t(\theta) \tilde{x}_t + \tilde{\vz}_t \in \bC^d, \quad t\in[n+1].
\end{equation}
Writing the above as a real-matrix equation, we obtain
\begin{align}
\label{eq:real-matrix-eqns}
   \vy_t \triangleq
    \begin{bmatrix}
    {\rm Re}(\tilde{\vy}_t) \\
     {\rm Im}(\tilde{\vy}_t)
    \end{bmatrix} = \begin{bmatrix}
        \operatorname{Re}(\tilde{\vh}_t(\theta)) & -\operatorname{Im}(\tilde{\vh}_t(\theta)) \\
        \operatorname{Im}(\tilde{\vh}_t(\theta)) & \operatorname{Re}(\tilde{\vh}_t(\theta))
    \end{bmatrix}
    \begin{bmatrix}
        \operatorname{Re}(\tilde{x}_t) \\
        \operatorname{Im}(\tilde{x}_t)
    \end{bmatrix}
     +
     \begin{bmatrix}
         \operatorname{Re}(\tilde{\vz}_t) \\
         \operatorname{Im}(\tilde{\vz}_t)
     \end{bmatrix} \triangleq \mH_t(\theta) \vx_t + \vz_t,
\end{align}
where $\vx_t \in \cX \subset \bR^2, \mH_t(\theta)\in \bR^{2d \times 2}, \vz_t, \vy_t \in \bR^{2d}$ which takes the form of the problem in Definition \ref{def:ice}.




% We specialize the estimation problem stated in Definition \ref{def:ice} to the wireless communication problems of interest. Consider a wireless channel with a single transmit antenna and $d$ receive antennae (see Fig. \ref{fig:TranEstimator}).


% Let $s_t \in \cX = \{x_I+ \sqrt{-1} \ x_Q  \mid x_I, x_Q\in\{\pm 1\}\}$ be the $t$th transmitted symbol.
% The transmit sequence $\{s_t\}$ is an i.i.d sequence of symbols drawn from $\cX$ with uniform probability.

% Let $\vy_t \in \bC^d$ be the received symbol vector, where $y^j_t$ denotes the received symbol at the $j$th antenna at time $t$. 
% Let $\vh_t(\theta) \in\bC^d$ be the wireless channel coefficient between the transmitter and the $j$th receiver antenna, and let $\vz_t$ be the additive noise at the receiver, at time $t$. 
% Then, we can write the input-output relation as
% \begin{equation}
% \label{eq:io_relation}
%     \vy_t = \vh_t(\theta) x_t + \vz_t, \quad t\in[\ell].
% \end{equation}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure below %%%%%%%%%%%%%
% \begin{figure}[ht]
% \centering
% \input{figures/TranEstimator}
% \caption{Notional diagram of a typical single-input multiple-output (SIMO) wireless channel combined with a transformer-based receiver}
% \label{fig:TranEstimator}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure above %%%%%%%%%%%%%

% For some $\sigma^2 > 0$, the sequence $\{\vz_t\}$ are independent and identically distributed (i.i.d.) Gaussian random vectors, with $\vz_{t, I},\vz_{t,Q}\sim \mathcal{N}(\mathbf{0}, \sigma^2 \mI_{d})$ for each $t\in[\ell]$. The ratio $1/\sigma^2$ is called the signal-to-noise-ratio (SNR).




% Next, we describe the latent context space $\Theta$, and the conditional distributions for the channel, i.e., $P_{h\mid \theta}$ for $\theta\in\Theta$. The channel parameter process $\{\vh_t(\theta)\}$ in the wireless communications typically depends on two aspects, discussed in the following subsections.




















% \begin{definition}
% \label{def:ice-subclass}
% {\bf (In-context estimation on the complex unit circle)} Estimate $\tilde{x} \in \cX \subset \bC$ from $\tilde{\vy} = \tilde{\vh}(\theta) \tilde{x} + \tilde{\vz} \in \bC^d$, and $n$ in-context examples $\tilde{\vy}_t = \tilde{\vh}(\theta) \tilde{x}_t + \tilde{\vz}_t$, $t\in [n]$, where $\tilde{\vh}(\theta)$ is a hidden variable independent of $\tilde{x}$, $\tilde{\vz}, \tilde{\vz}_t \stackrel{\rm iid}{\sim} \cC\cN(\0, \tilde{\bSigma}_{z})$ and $\tilde{x}, \tilde{x}_t \stackrel{\rm iid}{\sim} \cU(\cX)$, where $\cX \subset \bC$ is a finite subset of the unit circle in $\bC$, i.e., $\abs{z} = 1$ for any $z \in \cX$. We used the notation $\cU(\cX)$ to denote the uniform distribution over $\cX$.
% \end{definition}

% We remark that the above problem is the classical problem of estimating transmitted symbols from the received symbols in a wireless communication channel. To see the relation of the above problem with that in Definition \ref{def:ice-subclass}, first write the above as corresponding real-valued matrix equation:
% \begin{align}
% \label{eq:real-matrix}
%    \vy \triangleq
%     \begin{bmatrix}
%     \tilde{\vy}_I \\
%     \tilde{\vy}_Q
%     \end{bmatrix} = \begin{bmatrix}
%         \tilde{\vh}_I(\theta) & -\tilde{\vh}_Q(\theta) \\
%         \tilde{\vh}_Q(\theta) & \tilde{\vh}_I(\theta)
%     \end{bmatrix}
%     \begin{bmatrix}
%         \tilde{x}_I \\
%         \tilde{x}_Q
%     \end{bmatrix}
%      +
%      \begin{bmatrix}
%          \tilde{\vz}_I \\
%          \tilde{\vz}_Q
%      \end{bmatrix} \triangleq \mH(\theta) \vx + \vz,
% \end{align}
% where $\vz \sim \cN(\0, \bSigma_z)$ such that $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
%     \tilde{\bSigma}_z & \0 \\
%     \0 &  \tilde{\bSigma}_z
% \end{bmatrix}$, and note that $\bSigma_z^{-1} = 2 \begin{bmatrix}
%     \tilde{\bSigma}_{z}^{-1} & \0 \\
%     \0 &  \tilde{\bSigma}_{z}^{-1}
% \end{bmatrix}$.

% From now on, we only work with the above real quantities. Note that given $\mH$ the dependence of the estimation problem on $\theta$ vanishes. We next derive the minimum mean squared error (MMSE) estimate for $\vx$ given $\vy$ and $\mH$, by identifying $\cX \subset \bS^2$, the unit sphere in $\bR^2$.

% \begin{lemma}
% \label{lem:opt-MMSE-PSK}
% {\bf (MMSE estimate)}
%     The optimal estimator $\hat{\vx}_{\rm MMSE}: \bR^{2d} \times \bR^{2d\times 2} \to \bR^2$ for $\vx \in  \cX \subset \bS^2$ given $\vy \in \bR^{2d}, \mH \in \bR^{2d\times 2}$ where $\vy = \mH \vx + \vz$ for some $\vz \sim \cN(\0, \bSigma_z)$ is given by
%     \begin{align*}
%         \hat{\vx}_{\rm MMSE}(\vy, \mH; \bSigma_z, \cX) = \bE_{\vx \sim \cU(\cX), \vz \sim \cN(\0,\bSigma_z)}[\vx \mid \vy, \mH] = \frac{\sum_{\vx \in \cX}\vx \exp(\vy^T \bSigma_z^{-1} \mH \vx)}{\sum_{\vx \in \cX}\exp(\vy^T \bSigma_z^{-1} \mH \vx)},
%     \end{align*}
%     where $\mH \triangleq \begin{bmatrix}
%         \tilde{\vh}_I(\theta) & -\tilde{\vh}_Q(\theta) \\
%         \tilde{\vh}_Q(\theta) & \tilde{\vh}_I(\theta)
%     \end{bmatrix}$ for some $\tilde{\vh} = \tilde{\vh}_I + j \tilde{\vh}_Q \in \bC^d$, and $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
%         \tilde{\bSigma}_z & \0 \\
%         \0 & \tilde{\bSigma}_z
%     \end{bmatrix}$ for some symmetric positive definite matrix $\tilde{\bSigma}_z \in \bR^{d\times d}$.
% \end{lemma}

% \proof{It follows from elementary computations Bayes theorem (see Appendix \ref{sec:appendix-finite-estimation}).}

% Note that the above estimator assumes that the channel is perfectly known to the estimator. We emphasize that unlike the linear regression problem, even if the hidden variable is known to the estimator, the estimate for $\vx$ is still not perfect, in the sense that the estimation error is non-zero. We next consider a transformer to solve the above problem when $\vh$ is not known. Specifically, let $\mT^{\rm SA}_n$ be the output corresponding to the value of $\vx$ of a single layer softmax attention transformer (SAT) $\mT$ with the query, key matrices of the form $\tilde{\mW}_s = \begin{bmatrix} \mW_s & \0 \\ \0 & \0_{2\times 2}\end{bmatrix} \in \bR^{(2d+2)\times (2d+2)}$, $s = {\rm Q}, {\rm K}$, and the value matrix $\tilde{\mW}_{\rm V} = \begin{bmatrix}
%     \0 & \0 \\ \0 & \mI_2
% \end{bmatrix}$, acting on tokens $\vt_i \triangleq [\vy_i^T~\vx_i]^T \in \bR^{2d+2}$ for $i\in[n]$ and $\vt \triangleq [\vy^T~\0_2]^T \in \bR^{2d+2}$.  Denoting $\mW \triangleq \mW_{\rm Q}^T \mW_{\rm K}$, we can write the predicted value of $x$ by the transformer as
% \begin{align*}
%     \mT^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{\vx_i\}_1^n; \mW) = \frac{\sum_{i=1}^n \vx_i \exp(\vy^T \mW \vy_i) }{\exp(\vy^T \mW \vy) + \sum_{i=1}^{n} \exp(\vy^T \mW \vy_i)}.
% \end{align*}

% \begin{lemma}
% \label{lem:convergence-SA-PSK}
% {\bf (Functional form of asymptotic softmax attention)} For $i\in [n]$, if $\vx_i, \vy_i$ are such that $\vy_i = \mH \vx_i + \vz_i$, and $\vy = \mH \vx + \vz$, then we have
% \begin{align*}
%     \lim_{n \to \infty} \mT^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{\vx_i\}_1^n; \mW) = \frac{\sum_{\vx \in \cX}\vx \exp(\vy^T \mW \mH \vx)}{\sum_{\vx \in \cX}\exp(\vy^T \mW \mH \vx)} ~{\rm a.s.}
% \end{align*}
% \end{lemma}

% \proof{It follows by a careful application of the strong law of large numbers (see Appendix \ref{sec:appendix-finite-estimation}).}

% \begin{theorem}
% {\bf (Existence of a softmax attention estimator that is asymptotically optimal)} 
% \label{thm:opt-SA-PSK}
% There exists a softmax attention transformer such that it is asymptotically an optimal estimator in the mean squared error sense, i.e., a.s.
% \begin{align*}
%     \lim_{n\to \infty} \mT_n^{\rm SA}(\cdot; \bSigma_z^{-1}) = \hat{\vx}_{\rm MMSE}(\cdot; \bSigma_z, \cX)
% \end{align*}
% \end{theorem}
% \proof{It directly follows from Lemma \ref{lem:opt-MMSE-PSK} and Lemma \ref{lem:convergence-SA-PSK}.}

% Now that we proved existence, can the training such a transformer with long prompt length ($n\to\infty$) achieve the above optimal estimate?

% In order to answer the above question, we first define a training procedure as follows. Denote the $j$th prompt in the training data as $[\vt_1^j, \vt_2^j, \dots, \vt_n^j, \vt^j]$  for $j\in [p]$ such that $\vt_i^j = [(\vy_i^j)^T~(\vx_i^j)^T]^T, \vt^j =[(\vy^j)^T~(\vx^j)^T]^T \in \bR^{2d+2}, \vy_i^j = \mH^j \vx_i^j + \vz_i^j$, where $\vz^j, \vz_i^j \stackrel{\rm iid}{\sim} \bSigma_z, \vx^j, \vx_i^j \stackrel{\rm iid}{\sim} \cU(\cX)$ and $\mH^j \in \bR^{2d\times 2}$ is constructed from $\vh$ chosen from a distribution $\mu_\vh$.

% Let us define the pre-training loss of the transformer with the above training procedure as $\cL_n^p(\mW) \triangleq \frac{1}{p} \sum_{j=1}^p \norm{\mT_n^{\rm SA}(\vy^j, \{\vy_i^j\}_{i=1}^n, \{\vx_i^j\}_{i=1}^n; \mW)-\vx^j}_2^2$. We define the population loss as $\cL_n(\mW) \triangleq \lim_{p\to \infty} \cL_n^p(\mW)$. Thus, by the strong law of large numbers, $\cL_n(\mW) = \bE_{\vh\sim\mu_{\vh}, \bepsilon \sim \vz\sim\cN(\0, \bSigma_z), \vx, \vx_i \sim \cU(\cX)}[\norm{\mT_n^{\rm SA}(\vy, \{\vy_i\}_1^n, \{\vx_i\}_1^n; \mW)-\vx}_2^2]$ a.s., where the expectation is over the prompts in the pre-training distribution. We write the loss as $\cL_n(\mW; \mu_\vh, \bSigma_z, \cX)$ to indicate the dependence on the distribution of $\vh$, the input set $\cX$, and $\bSigma_z$ during the training. Finally, we define the asymptotic loss in the limit as $n\to\infty$ as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$, and write $\cL(\mW;\mu_\vh, \bSigma_z, \cX)$. Then, we have the following result:

% \begin{theorem}
% {\bf (Global minimizer)}
% \label{thm:global-min-PSK} For any pre-training distribution $\mu_\vh$ on the channel and inputs $\cX \subset \bS^2$, the matrix $\bSigma_z^{-1} \in \bR^{2d\times 2d}$ is the global minimizer of $\cL(\cdot; \mu_\vh, \bSigma_z, \cX)$.
% \end{theorem}
% \proof{It follows from the properties of conditional expectation, the uniform boundedness (in $n$) of $\mT_n^{\rm SA}(\cdot; \mW)$, and the dominated convergence theorem (see Appendix \ref{sec:appendix-finite-estimation}).}

% We remark that the optimality in Theorem \ref{thm:opt-SA-PSK} and Theorem \ref{thm:global-min-PSK} is only in the asymptotic limit. As such, the results are about expressiveness and the minimizer for a softmax attention transformer, akin to the results of a linear attention in \cite{bartlett} (barring convergence of the training procedure). Typically, we are interested in optimal  algorithms given $n$ examples. In particular, we are interested when $\tilde{\vh}(\theta)$ comes from a hierarchical distribution as $\theta \sim \bP_\Theta$ and then $\tilde{\vh} \sim \bP_{h\mid \theta}$. Here, the hidden context $\theta$ determines the right mixture from which $\tilde{\vh}(\theta)$ in the prompt is drawn from. For optimal estimators in the case of finite context length, the dependence on $\theta$ becomes important. In order to exploit this dependence, we next introduce multi-layer transformers as viable in-context estimator, and demonstrate its effectiveness. 


==> contents/introduction.tex <==
\section{Introduction}

Recent advances in our understanding of transformers ~\cite{NIPS2017_3f5ee243} have brought to the fore the notion that they are capable of in-context learning (ICL).  Here, a pre-trained transformer is presented with example prompts followed by a query to be answered of the form $(\vx_1,f(\vx_1, \theta), \hdots, \vx_k, f(\vx_k, \theta), \vx_{k+1}),$ where $\theta$ is a context common to all the prompts.  The finding is that the transformer is able to respond with a good approximation to $f(\vx_{k+1},\theta)$ for many function classes~\cite{garg2023transformers,panwar2024incontext}. 
The transformer itself is pre-trained, either implicitly or explicitly over a variety of contexts and so acquires the ability to generate in-distribution outputs conditioned on a specific context.

Although the interpretability of in-context learning for solving rich classes of problems can be very challenging, there have been attempts to understand the theoretical aspects of in-context learning for simpler problems, specifically linear regression. The work \cite{zhang2024trained} characterizes the convergence of the training dynamics of a single layer linear attention (LA) for solving a linear regression problem over random regression instances.
It shows that this configuration of the trained transformer is optimal in the limit of large prompt length. 

%\textcolor{red}{These paragraphs need some work.}
In this paper, we introduce an in-context estimation problem where
we are presented with the sequence $(g(\vx_1, \theta), \vx_1,\hdots,$ $g(\vx_k, \theta), \vx_k, g(\vx_{k+1}, \theta))$ where $g(\vx,\theta)$ is a stochastic function whose distribution is parameterized by $\theta$, and our goal is to estimate $\vx_{k+1}$. This inverse problem is inherently more challenging than predicting $f(\vx_{k+1}, \theta)$ for $\vx_{k+1}$ (as in linear regression) due to the complicated dependence of the optimal estimator on noisy observations.

The above formulation of in-context estimation models many problems of interest in engineering.
However, to keep the paper focused, we consider
a subclass of problems that is of particular interest to communication theory.
Here $\vx$ represents a sequence of transmitted symbols and the communication channel with the unknown state (context) $\theta$ maps $\vx$ 
into a sequence of received symbols 
represented by $\vy = f(\vx,\theta)$.
%with the communication channel mapping an input symbol $\vx$ to a received observation $\vy = g(\vx, \theta),$  with the addition of noise (details can be found in Section~\ref{sec:in-context-estimation}).
The receiver is then required to recover $\vx$ using in-context examples that can be constructed from the received symbols and transmitted pilot symbols.
More details about the function $f(\vx,\theta)$ and the in-context examples can be found in Section~\ref{sec:in-context-estimation}. 


Our work is motivated by the observation that a pre-trained transformer's ability to perform in-context sequence completion suggests strongly that it should be able to approximate the desired conditional mean estimator given the in-context examples for our inverse problem.  Essentially, if a transformer is pre-trained on a variety of contexts, it should be able to implicitly determine the latent context from pilot symbols and then perform end-to-end in-context estimation of transmitted symbols.  Once trained, such a transformer is simple to deploy because there are no runtime modifications, which could make it a potential building block of future wireless receivers. We indeed show this result both theoretically and empirically. 



% In this paper, we study the in-context estimation (ICE) ability of transformers. 
% \item We make a fundamental connection between the in-context learning property of transformers with our desire for in-context estimation applicable to communication systems.
    %\item For special cases of such problem (the symbols ($\{\vx_t\}_1^{k+1}$) are of constant magnitude), we theoretically show that there exists a configuration of single layer {\bf softmax attention transformer (SAT)} that it is asymptotically optimal.
%We prove the existence of a single layer SAT which is an optimal estimator in the mean squared error sense given an asymptotically long prompt, for a subset of ICE problems.

Our main contributions are:
\begin{itemize}
    \item We define the inverse problem of estimating symbols from noisy observations using in-context examples, which we term in-context estimation (ICE). This is more difficult than linear regression which is a well-studied in-context learning (ICL) problem.
    \item For special cases of such problems (detailed in Section \ref{sec:main_results}), we theoretically show that there exists a configuration of single layer {softmax attention transformer (SAT)} that is asymptotically optimal.
    \item We empirically demonstrate that multi-layer transformers are capable of efficiently solving representative ICE problems with finite in-context examples.
\end{itemize}

%\textcolor{red}{
%For special cases of such problem (the symbols ($\{\vx_t\}_1^{k+1}$) are of constant magnitude), we theoretically show that there exists a configuration of single layer {\bf softmax attention transformer (SAT)} that it is asymptotically optimal. - Is this not repeated in the second bullet item inside our significant contributions? Why not just say what our significant contributions are right here?}

% \textcolor{red}{
% The functional form of an SAT makes it a natural choice for the estimation problems (under Gaussian noise). - unless someone strongly feels this should be included, I would remove this sentence from the introduction.}
% \textcolor{blue}{This result is not implied by the earlier results on linear regression \cite{zhang2024trained}, \cite{ahn2024transformers} - can we move this statement to the prior work section?}

% \textcolor{red}{The following sentence has to be rephrased. It is not clear why the estimation error being bounded below makes it challenging. I think what you want to say is that the optimal estimator has a different form from that of the optimal estimate in the linear regression case. Therefore, the results in this paper are not implied by earlier results on linear regression.}

% It is important to remark that even this simpler problem is challenging in the sense that the estimation error is bounded below non-trivially (strictly positive lower bound).


%In a similar flavor, we work with a  and show that it is the right choice for in-context estimation problems.
%Here, 


%The context here corresponds to the communication channel physics, with the mobile velocity and receiver occlusion playing major roles in the specific channel evolution.


% While our theoretical understanding of such in-context learning in transformers is still in its infancy, their excellent empirical performance motivates us to explore the \emph{inverse problem} of in-context estimation.  Here, we are presented with the sequence $(f(\vx_1, \theta), \vx_1,\hdots,  f(\vx_k, \theta), \vx_k, f(\vx_{k+1}, \theta)),$ and are required to estimate $\vx_{k+1}.$  


%The prompt in the case of the communication problem is called \emph{pilot symbols}, which are symbols known in advance at the receiver.  A baseline approach towards estimating the transmitted symbol $\vx_{k+1}$ from the observation $\vy_{k+1}$ is to first estimate the channel function using the pilots, and then to estimate the transmitted symbol, conditioned on the channel estimate.  However, such an approach does not optimally exploit the relationship between the context, the channel function, and the received symbol.  
%The optimal estimator (in the mean squared error sense) computes the posterior mean estimate taking into account the full structure of the problem. However, the computational complexity of the optimal estimator is prohibitive. 





% We draw inspiration from wireless communication, 

%In this paper, we make a fundamental connection between the in-context learning property of transformers and in-context estimation for a certain type of problem pertinent to communication systems. 


% We show empirically that trained transformers perform estimation with a few in-context examples. Such estimators by transformers achieve the same performance as that of a context-aware estimator, suggesting that the transformer is able to learn the hidden context without a few examples.

% \textcolor{green}{
% This paragraph makes a good point, but does not flow well from the earlier paragraph. Can we find a sentence to connect the two ?}



% Our main results are to show that our connection is indeed accurate and that pre-trained transformers easily outperform the baseline algorithm, both for fixed and time-varying channels.  Furthermore, we observe that transformers are information-efficient. They come close to matching the performance of a genie-aided algorithm that conducts estimation with full knowledge of the latent context, suggesting that they are learning the optimal contextual inference function.  Thus, we demonstrate that transformers are well able to perform efficient in-context estimation.


==> contents/methodology.tex <==

\section{Methodology}

In this section, we describe the classical estimation techniques used to solve the estimation problem, along with a transformer model as an alternative.

\subsection{Context-aware and baseline estimators}
\label{baseline_genie_descriptions}
In this section, we describe some feasible context-aware estimators, that achieve a low MSE (close to that of \ref{eq:in_context_estimator}). For C1, $\theta = 0$, since the randomness of the channel parameter vector comes from a single random variable $\alpha$, the computation of the posterior mean involves an integral in one dimension. Hence, it can be computed in a computationally efficient manner. The exact expression appears in \ref{eq:one_ray_model_symbol_estimation}. 
In the remaining cases, we cannot evaluate the expression explicitly. In these cases, the context-aware estimator first computes the Linear Minimum Mean Square Estimate (LMMSE) $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$  of the channel parameter ${\vh}_{k+1}(\theta)$ given $S_k, \theta$. The exact details of computing the expression for $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$ are given in Appendix \ref{context_aware_estimators_derivation}. Incidentally, for $\theta=1$ in C1, and for all $\theta \in \Theta$ in C2, since $\vh_{k+1}(\theta)$ and $(\vy_t, t\in [k])$ are jointly Gaussian, conditioned on $(s_t, t\in[k])$, this channel estimate is in fact the minimum mean squared estimate (MMSE) of $\vh_{k+1}(\theta)$ given $S_k, \theta$. Then, the symbol is estimated by computing $\bE[s_{k+1} \mid \vh_{k+1}(\theta) = \hat{\vh}_{k+1}^{\rm LMMSE, \theta} \mid \vy_{k+1}]$; the exact expression for above conditional expectation is given in \ref{eq:symbol_estimate}.



For the context agnostic baseline, we describe an estimation procedure commonly used in the wireless communication. The estimator first computes the LMMSE of the channel (see Appendix \ref{baseline_for_agnostic_estimators}), which uses the correlation matrices corresponding to prior for the channel parameter process. Then, it estimates the symbol as the conditional mean, conditioned on the LMMSE for the channel. The exact details are given in Appendix \ref{baseline_for_agnostic_estimators}.

\subsection{Transformer} \label{training}
We train our transformer models as described in Section~\ref{in_context_estimation}. We follow the training setup used in \cite{ahuja2023incontext}, which is in turn based on the approach used in \cite{garg2023transformers}. For all experiments, we train a GPT-2 decoder-only model from scratch.

We specifically modify the setting in Section 4 of \cite{ahuja2023incontext}, regarding learning of functions sampled from a hierarchical distribution of function classes (``tasks"). In this setting, a task $\theta$ is sampled from some set of tasks $\Theta$, then a function $f$ is sampled from a set of functions $\mathcal{F}_\theta$ which is determined by $\theta$. In our case, $f$ is determined by the channel coefficients $\vh$, which we sample as described in Section~\ref{wireless_communication_problem}.

The training data is generated as follows. First we draw $\theta \sim {\rm Unif}(\Theta)$. In C1, we generate $\alpha \sim {\rm Unif}[0, \pi)$ and set $h^j_t(0) = \phi_j(\alpha)$. In C2, we generate the sequence $\vh^j = (h_t^j, t\in \bN)$ from a stationary Gaussian random process. For each training mini-batch, we re-sample $\theta$ and then independently sample each $\vh^j$.

As done in \cite{ahuja2023incontext}, we train our decoder models to perform prediction in the style of language models, where $$((\vy_1, \vx_1), (\vy_2, \vx_2), \dots, (\vy_k, \vx_k), \vy_{k+1})$$ are used to predict $\vx_{k+1}$. We use the sum of squared errors between all $(\vx_t, \hat{\vx}_t), t\in[k+1]$ as our loss function, where $\hat{\vx}_t =  T_W^{k+1}(S_k, \vy_{k+1})$. 

We set the number of antennae $d = 4$. For C2, we consider $M = 3$, where $v_1 = 5, v_2 = 15, v_3 = 30$ (all in m/s). These are representative of the typical values seen in practice for wireless communications. For C1, $\theta = 1$, we set $s = \lambda/4$. For C2, we use $f_c = 2.9 \times 10^9$ Hz, and $\lambda = f_c/c$, where $c = 3\times 10^8$ m/s is the speed of light. Further, we set the symbol duration $T_s =$ 1 millisecond in C2.

We include our model architecture details and other hyper-parameter settings in Appendix~\ref{parameters}.

==> contents/related-work-old.tex <==

\section{Related Work}
\subsection{Transformers and In-Context Learning}
Transformer architectures have become a popular model architecture across a variety of problems. The recent popularity of this architecture is in large part due to the fact that multi-head self-attention units have been shown to perform well on a wide variety of natural language tasks~\cite{NIPS2017_3f5ee243}.

In \cite{LanguageModelsAreFewShotLearners} it was shown that GPT-3, a transformer-based large language model, is able to perform well on novel, unseen tasks in a few-shot or zero-shot manner, known as in-context learning. The authors of \cite{xie2022an} used synthetic data to show that in-context learning can be interpreted as Bayesian inference, wherein a model first attempts to infer the task and then uses this prediction to carry out the task.

\cite{garg2023transformers} and \cite{ahuja2023incontext} are closely related to our work. In \cite{garg2023transformers}, the authors explore in-context learning from a different perspective than prior work. Rather than looking at in-context learning in the natural language setting, they pose this as the problem of learning to perform least-squares estimation for linear regression by being trained on sequence data. The authors of \cite{ahuja2023incontext} build on this work and provide mathematical theory to describe how this can be interpreted as the model performing Bayesian inference by estimating a posterior distribution.

Other work has gone further in explaining the mechanisms by which transformers are able to perform in-context learning. Some authors have explored the behavior of simplified transformer models on synthetic linear regression problems, as compared to the globally optimal solutions for these problems\cite{mahankali2023step,Zhang2023TrainedTL}.
In \cite{whatlearningalgorithm}, it is shown by construction that transformers can learn to fit a linear model at inference time given a context. This tells us that, at least in theory, transformers can learn to literally perform regression and related computations given some data. A related line of work explores the manner by which transformer models carry out these optimization procedures and shows that transformer models can perform nontrivial gradient-based optimization procedures at inference time\cite{von2023transformers,ahn2023transformers}. 
In \cite{EmergentICL}, the authors test how properties of training data impact in-context learning behaviors. 
The authors of \cite{min2022rethinking} similarly study how the properties of the context itself impact in-context learning performance. 

In summary, many different research directions have provided ways to interpret and understand in-context learning and the mechanisms by which transformer models do it. In our work, we primarily use the Bayesian perspective to view this ability and to understand how we can apply it to the wireless communication domain.

\subsection{Machine Learning for Wireless Communication}
The problem of symbol estimation in the presence of an unknown channel is a canonical problem in wireless communication and there is a large body of literature that considers model-driven traditional signal processing approaches. 
When the prior distribution for the channel follows a hierarchical model with latent contexts such as what we study in this paper, optimal model-based estimators become computationally infeasible. 
While approximations to the optimal estimators have been studied with restricted priors, the structure and performance of such estimators are highly dependent on the priors.






Recently, there has been significant interest in using machine learning methods such as variational inference \cite{ChannelEstimationUsingVAE}, \cite{UnsupervisedEqualizationUsingVAEs} and deep neural network models such as fully connected neural networks \cite{DeepLearningAidedChannelEstimation}, convolutional neural networks \cite{LearningMMSEChannelEstimator}, and recurrent neural networks \cite{RNNforChannelEstimation} 
for channel estimation and for symbol estimation \cite{aoudia2021end}. The authors of \cite{faycal} design an  end-to-end wireless communication system design using learning-based approach.
The work of \cite{neumann} provides a principled way of designing channel estimators in the setting of wireless communication, by training CNN-based neural network to efficiently estimate the channel parameters when it follows a hierarchical prior. The authors of \cite{UnsupervisedLinearAndNonLinearChannelEqAndDecoding} used variational autoencoders (VAEs) and unsupervised learning to implicitly learn and decode symbols in a wireless channel. In \cite{SemisupervisedVAEForNonLinearChannels}, the authors use VAEs in a semi-supervised setting to operate over non-linear channels. The approach in \cite{deepLearningForTimeVaryingMIMOChannels} uses a long short-term memory (LSTM) based channel parameter estimator for a time-varying channel. They are interested in learning the spatial correlation structure of the channel coefficients across the receiver antennae.
 
 
 The main distinction of our work from the previous works is that we make the connection between the in-context learning capabilities of the transformer and the symbol estimation problem in wireless communication. We show how the problem fits naturally in the setting, and provide empirical evidence that transformers achieve near-optimal performance. A comparative study of the performance of the transformers and other machine learning models is left for the future work.

==> contents/results-and-discussion.tex <==

\section{Results and discussion}

In this section, we present experimental results for scenarios 1 and 2. In short, across the scenarios we described, we show that GPT-2 models trained on sequences sampled from these scenarios are able to approach the performance of context-aware estimates. This is surprising, as the latter benchmark estimators are given the exact realization of $\theta$ for each case, while the models have to implicitly estimate this from the context in addition to predicting the symbols $\vx$.

\subsection{Scenario 1: Estimation under Time-invariant process}
We trained two GPT-2 models as described in Section~\ref{sec:training} on data sampled as per scenario~1. The only difference in training was the SNR used when sampling the data: we trained one model with an SNR of 0 dB and the other model with an SNR of -5 dB. In Figure~\ref{fig:ray_fading_results}, we present results for our trained models and our baseline methods on sequences from these two latent contexts. In these figures, for each context length $t$, we plot the MSE between the true $\vx_t$ and the predicted $\hat{\vx}_t$. 
We present these curves for the transformer model, context-aware estimate, and context-aware baseline (Section~\ref{baseline_genie_descriptions}).
We also plot a 90\% confidence interval for the transformer model's prediction errors.

%%%%%%%%%%%%%%%%%%%%%%%%% main plot below %%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/scenario1-combined-low-dpi.png}
    \caption{\small Estimation error in scenario 1 as a function of number of in-context examples. The performance of the transformer (red) is close to that of the optimal context-aware estimator (black)  while significantly outperforming a typical baseline (green) when latent context $\theta=0$.}
    \label{fig:ray_fading_results}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% main plot above %%%%%%%%%%%%%%

Let us first discuss the case with $\theta=0$. Here, even the zero-shot performance of the transformer model is better than the context-unaware model. This indicates that the model is able to use the statistics of the $\vy$ vectors to distinguish between $\theta=0$ and $\theta=1$. As the context length increases, for both SNR values, the transformer model performs better than the context-unaware baseline and approaches the performance of the lower-bound context-aware estimate. This shows that the model is able to determine the latent context and make a good estimate of the channel parameters, without being given any information beyond the $(\vy, \vx)$ pairs themselves.

When $\theta=1$, the three methods perform roughly the same across both SNR values and all context lengths. This is to be expected. The hidden parameter $\tilde{\vh}(1)$ in this case is Gaussian, and simply estimating the mean and variance of the channel will grant the best performance. The notable aspect of this inquiry is that the transformer model is able to correctly identify the context and has learned the correct way to estimate the channel for this context.

\subsection{Scenario 2: Estimation under Time-varying process}
We train the model on data generated as per scenario 2. We present results for this scenario in Figure~\ref{fig:time_varying}. These plots are produced in a manner similar to Figure~\ref{fig:ray_fading_results}, with the added challenge that the hidden parameters $\tilde{\vh}_t(\theta)$ vary with time $t$.



%%%%%%%%%%%%%%%%%%%%%%%%% main plot below %%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/scenario2-combined-SNR0-low-dpi.png}
    \caption{\small Estimation error in scenario 2 as a function of number of in-context examples. The transformer (red) computes the optimal estimator (orange) with its performance approaching the context-aware estimator (black) as the number of examples increases, while significantly outperforming typical baselines (green, blue) for latent contexts $\theta=15, 30$.}
    \label{fig:time_varying}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% main plot above %%%%%%%%%%%%%%

In Figure~\ref{fig:time_varying}, we can see that the transformer model and other estimators have an MSE of 2 with zero examples for every $\theta$.
Because the distribution of the noise $\vz_1$ and the parameter $\tilde{\vh}_1(\theta)$ is symmetric about $\0$, any model requires at least one $(\vy, \vx)$ pair before it is able to make a meaningful prediction. 

Across all $\theta$, the performance of the transformer-based estimator matches the performance of the context-unaware estimator ${\rm CME}[x \mid {\rm MMSE}[h]]$ at every context length. As the context length increases both these estimates approach the performance of the context-aware estimator. This indicates that, with enough examples, the model is able to estimate the latent context $\theta$ and the hidden parameters $\tilde{\vh}_t(\theta)$, although the process is time-varying. There is a significant gap between the performance of the context-unaware baseline methods ${\rm CME}[x \mid {\rm MMSE}[h]]$, ${\rm CME}[x \mid {\rm LMMSE}[h]]$  and the performance of the other methods, demonstrating that performing well on this problem requires knowing or estimating $\theta$ well. The transformer model is able to accurately infer the context and use this information to perform nearly as well as the context-aware estimator.


==> contents/softmax-attention-theory.tex <==

\section{Main Results}
\label{sec:main_results}
In this section, we present our theoretical analysis for a single layer softmax attention transformer (SAT) as an estimator for the problem corresponding to \eqref{eq:complex-est-prob}.
We work with the following assumption.
\begin{assumption}
\label{assum:SIMO-model} The distributions of the hidden process, input symbols, and noise are characterized as follows.
\begin{enumerate}[label=(\alph*)]
    \item The hidden process is time invariant, i.e., $\tilde{\vh}_t(\theta) = \tilde{\vh}(\theta)$, where $\tilde{\vh}(\theta) \sim \bP_{h\mid \theta}$ is a \emph{fixed} hidden variable under the context $\theta \sim \bP_\Theta$.
    \item The inputs $\tilde{x}_t \stackrel{\rm iid}{\sim} \bP_x$ where $\bP_x$ is some distribution on $\tilde{\cX}$, and $\tilde{\cX} \subset \bC$ is a finite subset of the unit circle in $\bC$, i.e., $\abs{z} = 1$ for any $z \in \tilde{\cX}$. 
    \item The noise samples $\tilde{\vz}_t \stackrel{\rm iid}{\sim} \cC\cN(\0, \tilde{\bSigma}_{z})$ for some real positive definite matrix $\tilde{\bSigma}_z \in \bR^{d\times d}$.
\end{enumerate}
\end{assumption}

Then, the real equations are given by
\begin{equation}
\label{eq:real-constant-h}
    \vy_t = \mH(\theta) \vx_t + \vz_t, \quad t\ge 1
\end{equation}
 where $\vz_t \sim \cN(\0, \bSigma_z)$ such that $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
    \tilde{\bSigma}_z & \0 \\
    \0 &  \tilde{\bSigma}_z
\end{bmatrix}$, and note that $\bSigma_z^{-1} = 2 \begin{bmatrix}
    \tilde{\bSigma}_{z}^{-1} & \0 \\
    \0 &  \tilde{\bSigma}_{z}^{-1}
\end{bmatrix}$, and $\vx_t \in \cX$ can be identified as a subset of unit sphere $\bS^2$ in $\bR^2$. From now on, we only work with the above real quantities. 

We next derive the minimum mean squared error (MMSE) estimate for $\vx_t$ given $\vy_t$ and $\mH_t = \mH$.
Note that when $\mH_t = \mH$ is known, the dependence of the estimation problem on $\theta$ vanishes.
Further, $\left\{ (\vy_t, \vx_t) \right\}$ are conditionally independent and identically distributed (iid) given $\mH_t = \mH$ for all $t$. Therefore, the MMSE estimation corresponds to estimating $\vx$ from $\vy = \mH \vx + \vz$ when $\mH$ is known.

\begin{lemma}
\label{lem:opt-MMSE-PSK}
{\bf (MMSE estimate)}
    The optimal estimator $\hat{\vx}^{\rm MMSE}: \bR^{2d} \times \bR^{2d\times 2} \to \bR^2$ for $\vx \in  \cX \subset \bS^2$ given $\vy \in \bR^{2d}, \mH \in \bR^{2d\times 2}$ where $\vy = \mH \vx + \vz$ for some $\vz \sim \cN(\0, \bSigma_z)$ is given by
    \begin{align*}
        \hat{\vx}^{\rm MMSE}(\vy, \mH; \bSigma_z, \bP_x) = \bE[\vx \mid \vy, \mH] = \frac{\sum_{\vx \in \cX}\vx \bP_x(\vx) \exp(\vy^T \bSigma_z^{-1} \mH \vx)}{\sum_{\vx \in \cX}  \bP_x(\vx) \exp(\vy^T \bSigma_z^{-1} \mH \vx)},
    \end{align*}
    where $\mH \triangleq \begin{bmatrix}
        \operatorname{Re}(\tilde{\vh}) & -\operatorname{Im}(\tilde{\vh}) \\
        \operatorname{Im}(\tilde{\vh}) & \operatorname{Re}(\tilde{\vh})
    \end{bmatrix}$ for some $\tilde{\vh} \in \bC^d$, and $\bSigma_z \triangleq \frac{1}{2} \begin{bmatrix}
        \tilde{\bSigma}_z & \0 \\
        \0 & \tilde{\bSigma}_z
    \end{bmatrix}$ for some symmetric positive definite matrix $\tilde{\bSigma}_z \in \bR^{d\times d}$.
\end{lemma}

\proof{This follows from elementary computations involving Bayes theorem (see Appendix~\ref{sec:appendix-finite-estimation}).}

Since $\mH(\theta)$ is not known in the problems we consider, the above estimator essentially provides a lower bound on the performance of any in-context estimator. 

Let us consider a single layer softmax attention transformer (SAT) to solve the in-context estimation of $\vx$ given observation $\vy$ and $n$ in-context examples $\cP^n_\theta \triangleq \{(\vy_t, \vx_t), t\in[n]\}$, where $(\vy, \vx)$ and $(\vy_t, \vx_t)$ in $\cP_\theta^n$ satisfy \eqref{eq:real-constant-h}. 
Let $\mT^{\rm SA}$ denote an SAT with the query, key, and value matrices $\tilde{\mW}_Q, \tilde{\mW}_K, \tilde{\mW}_V$ respectively, acting on $(n+1)$ tokens $\vu_t \triangleq [\vy_t^T~\vx_t^T]^T \in \bR^{2d+2}$ for $t\in[n]$ and $\vu_{n+1} \triangleq [\vy^T~\0_2^T]^T \in \bR^{2d+2}$. Let $\mU_{n+1}$ be the matrix with columns $\vu_t$ for $t\in[n+1]$. Then, the $(n+1)$th output token is given by
\begin{align}
\label{eq:transformer-output}
    \mT_{n+1}^{\rm SA}(\mU_{n+1}) = \frac{\sum_{t=1}^{n+1} \tilde{\mW}_V \vu_t \exp(\vu_{n+1}\tilde{\mW}_Q^T \tilde{\mW}_K \vu_t)}{\sum_{t=1}^{n+1} \exp(\vu_{n+1}\tilde{\mW}_Q^T \tilde{\mW}_K \vu_t)}.
\end{align}

% The estimate of the above SAT for $\vx$ is provided by the last two entries in the $(n+1)$th output token, i.e., $[\mT_{n+1}^{\rm SA}]_{2d+1:2d+2}$. We denote this estimate with $n$ examples as $\hat{\vx}_{\rm SA}^n$.

The estimate of the SAT for \(\vx\) using \(n\) examples, denoted by \(\hat{\vx}^{\rm SA}_{n}\)  is obtained from the last two elements of the \((n+1)\)th output token, i.e., \([\mT_{n+1}^{\rm SA}]_{2d+1:2d+2}\).
Thus, the first $n$ columns of $\tilde{\mW}_V$ do not affect the output $\hat{\vx}^{\rm SA}_{n}$, hence we set them to zeros without loss of generality. Motivated by the form of the MMSE estimate, we choose to re-parameterize the remaining entries of the weights as below:
\begin{align}
\label{eq:query-key-values}
    \tilde{\mW}_Q = \begin{bmatrix} \mW_Q & \0_{2d\times 1} \\ \0_{1\times 2d} & \0_{2\times 2}\end{bmatrix}, \quad \tilde{\mW}_K = \begin{bmatrix} \mW_K & \0_{2d\times 1} \\ \0_{1\times 2d} & \0_{2\times 2}\end{bmatrix}, \quad \tilde{\mW}_V = \begin{bmatrix}
    \0_{2d\times 2d} & \0_{2d\times 1} \\ \0_{1\times 2d} & \mI_2
\end{bmatrix}.
\end{align}

Denoting $\mW \triangleq \mW_{\rm Q}^T \mW_{\rm K} \in \bR^{2d\times 2d}$, using \eqref{eq:query-key-values} in \eqref{eq:transformer-output}, we get
\begin{align*}
    \hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW) = \frac{\sum_{t=1}^n \vx_t \exp(\vy^T \mW \vy_t) }{\exp(\vy^T \mW \vy) + \sum_{t=1}^{n} \exp(\vy^T \mW \vy_t)}.
\end{align*}

\begin{lemma}
\label{lem:convergence-SA-PSK}
{\bf (Functional form of asymptotic softmax attention)}
For any $\theta \in \Theta$, suppose $\mH_i(\theta) = \mH$ is the common hidden parameter for $i \in [n+1]$, such that $\vy_i = \mH \vx_i + \vz_i$, and $\vy = \mH \vx + \vz$.
For a prompt $\mU_{n+1}$ with the $t$th column constructed as 
$\vu_t \triangleq [\vy_t^T, \vx_t^T]^T$ for $t\in[n]$ and $\vu_{n+1} \triangleq [\vy^T, \0_2^T]^T$, the estimated value by the transformer $\hat{\vx}_n^{\rm SA}$ with parameter $\mW$ satisfies
\begin{align*}
    \lim_{n \to \infty} \hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW) = \frac{\sum_{\vx \in \cX}\vx  \bP_x(\vx) \exp(\vy^T \mW \mH \vx)}{\sum_{\vx \in \cX}  \bP_x(\vx) \exp(\vy^T \mW \mH \vx)} ~{\rm a.s.}
\end{align*}
\end{lemma}

\proof{This follows by a careful application of the strong law of large numbers (see Appendix \ref{sec:appendix-finite-estimation}).}

\begin{theorem}
{\bf (Existence of a softmax attention estimator that is asymptotically optimal)} 
\label{thm:opt-SA-PSK}
%There exists a softmax attention transformer such that it is asymptotically an optimal estimator in the mean squared error sense, i.e., a.s.
There exists a softmax attention transformer such that, for any asymptotically long prompt, its estimate converges to the optimal MMSE estimator, i.e.,
\begin{align*}
     \lim_{n \to \infty} \hat{\vx}^{\rm SA}_{n}(\cdot; \bSigma_z^{-1}) = \hat{\vx}^{\rm MMSE}(\cdot; \bSigma_z, \bP_x) \quad \text{a.s.}
\end{align*}
\end{theorem}
\proof{This result follows directly from Lemma \ref{lem:opt-MMSE-PSK} and Lemma \ref{lem:convergence-SA-PSK}.}

This establishes the fact that the single layer softmax attention transformer architecture is expressive enough to asymptotically achieve optimal performance.
We then turn to the training process: can the training of such a transformer with (asymptotically) long prompt length achieve optimal performance?

To begin answering this question, we define the training procedure as follows.
Let prompt $j\in [n_p]$ in the training data be $\mU^j_{n+1}$ with columns $[\vu_1^j, \vu_2^j, \dots, \vu_n^j, \vu^j]$; therein, $\vu_i^j = [(\vy_i^j)^T~(\vx_i^j)^T]^T$, $\vu^j = [(\vy^j)^T~(\vx^j)^T]^T \in \bR^{2d+2}$, $\vy_i^j = \mH^j \vx_i^j + \vz_i^j$, where $\vz^j, \vz_i^j \stackrel{\rm iid}{\sim} \cN(\0,\bSigma_z)$, $\vx^j, \vx_i^j \stackrel{\rm iid}{\sim} \bP_x(\cX)$, and $\mH^j \in \bR^{2d\times 2}$ is constructed from $\tilde{\vh}$ chosen from a distribution $\bP_{h\mid \theta}$ for some $\theta \sim \bP_\Theta$.

Let us define the pre-training loss of the transformer as
\begin{equation*}
    \cL_n^{n_p}(\mW) \triangleq \textstyle \frac{1}{n_p} \sum_{j=1}^{n_p} \norm{\hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW)-\vx^j}_2^2 .
\end{equation*}
We define the population loss as $\cL_n(\mW) \triangleq \lim_{n_p\to \infty} \cL_n^{n_p}(\mW)$. Thus, by the strong law of large numbers, $\cL_n(\mW) = \bE_{\theta \sim \bP_\Theta, \tilde{\vh} \sim \bP_{h\mid \theta}, \vz\sim\cN(\0, \bSigma_z), \vx, \vx_i \sim \bP_x}[\norm{\hat{\vx}^{\rm SA}_{n}(\mU_{n+1}; \mW)-\vx}_2^2]$ a.s., where the expectation is over the prompts in the pre-training distribution. We write the loss as $\cL_n(\mW; \bSigma_z, \bP_x, \bP_{\Theta,h})$ to indicate the dependence on the distribution of $\vh$, the input set $\cX$, and $\bSigma_z$ during the training. Finally, we define the asymptotic loss in the limit as $n\to\infty$ as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$, and write $\cL(\mW; \bSigma_z, \bP_x, \bP_{\Theta,h})$.

\begin{theorem}
{\bf (Global minimizer)}
\label{thm:global-min-PSK} For any pre-training distribution $\bP_{\Theta, h}$ on the latent context of the hidden parameters, and any distribution of the inputs $\bP_x$, the matrix $\bSigma_z^{-1} \in \bR^{2d\times 2d}$ is the global minimizer of $\cL(\cdot; \bSigma_z, \bP_x, \bP_{\Theta,h})$.
\end{theorem}
\proof{It follows from the properties of conditional expectation, the uniform boundedness (in $n$) of $\hat{\vx}^{\rm SA}_{n}(\cdot; \mW)$, and the dominated convergence theorem (see Appendix \ref{sec:appendix-finite-estimation}).}

We remark that the optimality in Theorem \ref{thm:opt-SA-PSK} and Theorem \ref{thm:global-min-PSK} is only in the asymptotic limit. As such, the results are about the expressiveness and the minimizer of the training loss for a softmax attention transformer, akin to the results of linear attention in \cite{zhang2024trained} (barring convergence of the training procedure). Typically, we are interested in optimal algorithms given $n$ examples. For optimal estimators in the case of finite context length, the dependence on $\theta$ becomes important. To exploit this dependence, we next introduce multi-layer transformers as viable in-context estimators and demonstrate their effectiveness. 


==> contents/softmax-for-BPSK.tex <==
\section{Softmax Attention}

\begin{problem}
{\bf (In-context estimation)}
\label{pr:ice}
    Estimate $x$ from $\vy = \vh x + \bepsilon$ and $n$ in-context examples (pilots) $\{(\vy_i, x_i)\}_1^n$ that satisfy $\vy_i = \vh x_i + \bepsilon_i$ where $\vh \in \bR^d$ is a fixed hidden variable (channel) and  $\bepsilon, \bepsilon_i \stackrel{\rm iid}{\sim} \cN(\0, \bSigma_{\bepsilon})$, $x, x_i \stackrel{\rm iid}{\sim} \cU\{\pm 1\}$.
\end{problem}

First, we derive the minimum mean squared error (MMSE) estimate for $x$ given $\vy$ and the hidden variable $\vh$.

\begin{lemma}
\label{lem:opt-MMSE}
{\bf (MMSE estimate)}
    The optimal estimator $\hat{x}_{\rm MMSE}: \bR^d \times \bR^d \to \bR$ for the transmitted symbol $x$ given $\vy, \vh$ where $\vy = \vh x + \bepsilon$ for some $\bepsilon \sim \cN(\0, \bSigma_{\bepsilon})$ is given by
    \begin{align*}
        \hat{x}_{\rm MMSE}(\vy, \vh; \bSigma_{\bepsilon}) = \bE_{x, \bepsilon}[x \mid \vy, \vh] = \tanh(\vy^T\bSigma_{\bepsilon}^{-1}\vh).
    \end{align*}
\end{lemma}
\proof{It follows from elementary computations involving Bayes theorem (see Appendix \ref{sec:appendix}). }

Note that the above estimator assumes that the channel is perfectly known to the estimator. Unlike the linear regression problem, even if the hidden variable is known to the estimator, the estimate for $x$ is still not perfect, in the sense that the estimation error is non-zero. We next consider a transformer to solve the above problem when $\vh$ is not known. Specifically, let $T^{\rm SA}$ be a single layer softmax attention (SA) transformer $T$ with the query, key matrices of the form $\tilde{\mW}_s = \begin{bmatrix} \mW_s & \0 \\ \0 & 0\end{bmatrix}$, $s = {\rm Q}, {\rm K}$, and the value matrix $\tilde{\mW}_{\rm V} = \begin{bmatrix}
    \0 & \0 \\ \0 & 1
\end{bmatrix}$, acting on tokens $\vt_i \triangleq [\vy_i^T~x_i]^T \in \bR^{d+1}$ for $i\in[n]$ and $\vt \triangleq [\vy^T~0]^T \in \bR^{d+1}$.  Denoting $\mW \triangleq \mW_{\rm Q}^T \mW_{\rm K}$, we can write the predicted value of $x$ by the transformer as
\begin{align*}
    T^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n; \mW) = \frac{\sum_{i=1}^n x_i \exp(\vy^T \mW \vy_i) }{\exp(\vy^T \mW \vy) + \sum_{i=1}^{n} \exp(\vy^T \mW \vy_i)}.
\end{align*}


\begin{lemma}
\label{lem:convergence-SA}
{\bf (Functional form of asymptotic softmax attention)} For $i\in [n]$, if $x_i, \vy_i$ are such that $\vy_i = \vh x_i + \bepsilon_i$, and $\vy = \vh x + \bepsilon$, then we have
\begin{align*}
    \lim_{n \to \infty} T^{\rm SA}_n(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n;  \mW) = \tanh(\vy^T \mW \vh)~{\rm a.s.}
\end{align*}
\end{lemma}

\proof{It follows by a careful application of the strong law of large numbers (see Appendix \ref{sec:appendix}).}

\begin{theorem}
{\bf (Existence of a softmax attention estimator that is asymptotically optimal)} 
\label{thm:opt-SA}
There exists a softmax attention transformer such that it is asymptotically an optimal estimator in the mean squared error sense, i.e.,
\begin{align*}
    \lim_{n\to \infty} T_n^{\rm SA}(\cdot; \bSigma_{\bepsilon}^{-1}) = \hat{x}_{\rm MMSE}(\cdot; \bSigma_{\bepsilon})
\end{align*}
\end{theorem}
\proof{It directly follows from Lemma \ref{lem:opt-MMSE} and Lemma \ref{lem:convergence-SA}.}

Now that we proved existence, can the training such a transformer with $n\to\infty$ achieve the above optimal estimate?


In order to answer the above question, we first define a training procedure as follows. Denote the $j$th prompt in the training data as $[\vt_1^j, \vt_2^j, \dots, \vt_n^j, \vt^j]$  for $j\in [p]$ such that $\vt_i^j = [(\vy_i^j)^T~x_i^j]^T, \vt=[(\vy^j)^T~x^j]^T \in \bR^{d+1}, \vy_i^j = \vh^j \vx_i^j + \bepsilon_i^j$, where $\bepsilon^j, \bepsilon_i^j \stackrel{\rm iid}{\sim} \bSigma_{\bepsilon}, x^j, x_i^j \stackrel{\rm iid}{\sim} \cU\{\pm 1\}$ and $\vh^j \in \bR^d$ can be chosen from a distribution $\mu_\vh$.


Let us define the pre-training loss of the transformer with the above training procedure as $\cL_n^p(\mW) \triangleq \frac{1}{p} \sum_{j=1}^p (T_n^{\rm SA}(\vy^j, \{\vy_i^j\}_{i=1}^n, \{x_i^j\}_{i=1}^n; \mW)-x^j)^2$. We define the population loss as $\cL_n(\mW) \triangleq \lim_{p\to \infty} \cL_n^p(\mW)$. Thus, by the strong law of large numbers, $\cL_n(\mW) = \bE_{\vh\sim\mu_{\vh}, \bepsilon \sim \cN(\0, \bSigma_{\bepsilon}), x, x_i \sim \cU\{\pm 1\}}[(T_n^{\rm SA}(\vy, \{\vy_i\}_1^n, \{x_i\}_1^n; \mW)-x)^2]$ a.s., where the expectation is over the prompts in the pre-training distribution. We write the loss as $\cL_n(\mW; \mu_\vh, \bSigma_{\epsilon})$ to indicate the dependence on the distribution of $\vh$ and $\bepsilon$ during the training. Finally, we define the asymptotic loss in the limit as $n\to\infty$ as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$, and write $\cL(\mW;\mu_\vh, \bSigma_{\bepsilon})$. Then, we have the following result.
\begin{theorem}
{\bf (Global minimizer)}
\label{thm:global-min} For any $\mu_\vh$, $\mW^* = \bSigma_{\bepsilon}^{-1}$ is the global minimizer of $\cL(\cdot; \mu_\vh, \bSigma_{\bepsilon})$.
\end{theorem}
\proof{It follows from the properties of conditional expectation, the uniform boundedness (in $n$) of $T_n^{\rm SA}(\cdot; \mW)$, and the dominated convergence theorem (see Appendix \ref{sec:appendix}).}





% \subsection{Convergence of estimate by softmax attention to conditional mean estimate}

% Let $P(y=+1) = P(y=-1) = 1/2$. Given $\vh$, the MMSE estimate of $y$ from $\vx = \vh y + \vz$ where $\vz \sim \cN(0,\bSigma)$ is given  the conditional mean estimate (CME) as
% \begin{align*}
%     y^{\rm CME}(\vx,\vh;\bSigma) = \bE[y \mid \vx, \vh] 
%     &= P(y=1 \mid \vx,\vh)-P(y=-1 \mid \vx,\vh) \\
%     &= \frac{P(y=1) P(\vx,\vh \mid y=1)}{P(\vx,\vh)} -\frac{P(y=-1) P(\vx,\vh \mid y=-1)}{P(\vx,\vh)} \\
%     &= \frac{ P(y=+1) P(\vx, \vh \mid y=1) - P(y=-1) P(\vx, \vh \mid y=-1)}{ P(y=+1) P(\vx, \vh \mid y=1) + P(y=-1) P(\vx, \vh \mid y=-1)} \\
%     &= \frac{P(\vz = \vx-\vh) - P(\vz=\vx+\vh)}{P(\vz = \vx-\vh) + P(\vz=\vx+\vh)} \\
%     &= \frac{\exp(-\frac{1}{2}(\vx-\vh)^T \bSigma^{-1}(\vx-\vh))-\exp(-\frac{1}{2}(\vx+\vh)^T \bSigma^{-1}(\vx+\vh))}{\exp(-\frac{1}{2}(\vx-\vh)^T \bSigma^{-1}(\vx-\vh))+\exp(-\frac{1}{2}(\vx+\vh)^T \bSigma^{-1}(\vx+\vh))} \\
%     &= \frac{1-\exp(-\frac{1}{2} ((\vx+\vh)^T \bSigma^{-1}(\vx+\vh)-(\vx-\vh)^T \bSigma^{-1}(\vx-\vh)))}{1+\exp(-\frac{1}{2} ((\vx+\vh)^T \bSigma^{-1}(\vx+\vh)-(\vx-\vh)^T \bSigma^{-1}(\vx-\vh)))} \\
%     &= \frac{1-\exp(-\frac{1}{2}(4\vx^T\bSigma^{-1}\vh))}{1+\exp(-\frac{1}{2}(4\vx^T\bSigma^{-1}\vh))} = \tanh(\vx^T\bSigma^{-1}\vh) = \frac{\exp(\vx^T\bSigma^{-1}\vh)-\exp(-\vx^T\bSigma^{-1}\vh)}{\exp(\vx^T\bSigma^{-1}\vh)+\exp(-\vx^T\bSigma^{-1}\vh)}.
% \end{align*}

% \subsubsection{Under balanced inputs in the prompt}
% For the softmax attention, for the ease of notation we denote $\vx_{N+1}$ as $\vx$ and $y_{N+1}$ as $y$. For $N=2n$ assume that we have balanced inputs, i.e., $y_i = +y$ and $y_{n+i} = -y$ for $i\in[n]$. Hence, we have $\vx_i = \vh y + \vz_{i}, \vx_{n+i} = -\vh y + \vz_{n+i}$, for $i\in[n]$. Then, for $\mW = \bSigma^{-1}$ we can write the output of the softmax attention as
% \begin{align*}
%     &y^{\rm SA}_{n}(\vx,\{y_i\},\{\vx_i\}; \mW) \triangleq y \frac{\sum_{i=1}^n \exp(\vx^T\mW\vx_i) - \sum_{i=1}^n \exp(\vx^T \mW\vx_{n+i})}{\exp(\vx^T\mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW\vx_i) + \sum_{i=1}^n \exp(\vx^T \mW\vx_{n+i})} \\
%     &\hspace{2pt} = y\frac{\frac{1}{n} \sum_{i=1}^n \exp((\vx^T\mW(\vh y +\vz_i))) - \frac{1}{n}\sum_{i=1}^n \exp((\vx^T\mW(-\vh y +\vz_{n+i}))}{ \frac{1}{n}\exp(\vx^T\mW \vx) + \frac{1}{n} \sum_{i=1}^n \exp((\vx^T\mW(\vh y +\vz_i))) + \frac{1}{n}\sum_{i=1}^n \exp((\vx^T\mW(-\vh y +\vz_i)))} \\
%     &\hspace{2pt} = y\frac{\exp(\vx^T\mW\vh y)(\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_i)) - \exp(-\vx^T\mW\vh y) (\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW^{-1}\vz_{n+i}))}{\frac{1}{n}\exp(\vx^T\mW\vx)+\exp(\vx^T\mW\vh y)(\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_i)) + \exp(-\vx^T\mW\vh y) (\frac{1}{n} \sum_{i=1}^n \exp( \vx^T\mW\vz_{n+i}))}.
% \end{align*}
% For any given $\vx,\vh \in \bR^d$ (denote $\bE[\cdot \mid \vx]$ as $\bE[\cdot]$), $\xi_j \triangleq \vx^T \mW\vz_j = 0$ are iid Gaussian random variables with mean $\bE[\xi_1]  = \vx^T\mW\bE[\vz_1] = 0$, and variance $\bE[\vx^T \mW \vz_1 \vz_1^T \mW^T \vx] = \vx^T \mW\bSigma\mW^T\vx \triangleq \gamma(\vx)$. We call $\gamma(\vx)$ the instantaneous SNR. Hence, $\xi_j \stackrel{\rm iid}{\sim}  \cN (0, \gamma(\vx))$, $j\ge 1$. Therefore, $\zeta_j \triangleq \exp(\xi_j)$ are iid log-normal random variables with parameters $\mu_0 \triangleq 0, \sigma_0^2 \triangleq \gamma(\vx)$ with mean and variance given by $\bE[\zeta_1] = \exp(\mu_0 + \sigma_0^2/2) = \exp(\gamma(\vx)/2)$, and ${\rm Var}(\zeta_1) = (\exp(\sigma_0^2)-1)\exp(2\mu_0 + \sigma_0^2) = (\exp(\gamma(\vx))-1)\exp(\gamma(\vx)) < \infty$. Hence, by the strong law of large numbers $\frac{1}{n}\sum_{i=1}^n \zeta_i \to \bE[\zeta_1]$ a.s. Therefore, by continuity, for any $\vx,\{y_i\}, \{\vx_i\}$, we get $y^{\rm SA}_{n}(\vx,\{y_i\},\{\vx_i\}; \mW) \to y \frac{\bE[\zeta_1]\exp(\vx^T\mW\vh)-\bE[\zeta_1]\exp(-\vx^T\mW\vh)}{\bE[\zeta_1]\exp(\vx^T\mW\vh)+\bE[\zeta_1]\exp(-\vx^T\mW\vh)} = \frac{\exp(\vx^T\mW\vh)-\exp(-\vx^T\mW\vh)}{\exp(\vx^T\mW\vh)+\exp(-\vx^T\mW\vh)} \triangleq \tanh(\vx^T\mW\vh)$ a.s. for any $\bSigma \succ 0, \vh,\vx\in\bR^d$.
% When $n$ is large, then the output of the transformer is ${y}^{\rm SA}(\cdot; \mW) = \tanh(\vx^T\mW\vh) = y^{\rm CME}(\cdot ; \mW)$.

% \subsubsection{Arbitrary inputs}

% Let $\{y_i\}_1^n \stackrel{\rm iid}{\sim} {\rm Unif}(\pm 1), \{\vz_i\}_1^n \stackrel{\rm iid}{\sim} \cN(\0, \bSigma)$, and $\vx_i = \vh y_i + \vz_i$ for $i\in[n]$. Denote $I_n^+ \triangleq \{i \in [n]: y_i = y\}$, and $I_n^{-} \triangleq [n] \setminus I_n^{+}$. Then, the output of the softmax attention can be written as
% \begin{align*}
%     &y_n^{\rm SA}(\vx,\{\vx_i\}_1^n,\{y_i\}_1^n;\mW)
%     = \frac{\sum_{i=1}^n y_i \exp(\vx^T \mW \vx_i)}{\exp(\vx^T \mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW \vx_i)} \\
%     &= y\frac{\exp(\vx^T\mW \vh y) \frac{\abs{I_n^+}}{n} \frac{1}{\abs{I_n^{+}}}\sum_{i\in I_n^{+}} \exp(\vx^T\mW \vz_i) -  \exp(-\vx^T\mW \vh y) \frac{\abs{I_n^-}}{n} \frac{1}{\abs{I_n^{-}}} \sum_{i\in I_n^{-}} \exp(\vx^T \mW \vz_i)}{\frac{1}{n}\exp(\vx^T \mW \vx) + \frac{\abs{I_n^+}}{n} \frac{1}{\abs{I_n^{+}}} \exp(\vx^T\mW \vh y) \sum_{i\in I_n^{+}} \exp(\vx^T\mW \vz_i) + \frac{\abs{I_n^-}}{n} \frac{1}{\abs{I_n^{-}}} \exp(-\vx^T\mW \vh y)\sum_{i\in I_n^{-}} \exp(\vx^T \mW \vz_i)}
% \end{align*}
% By the strong law of large numbers, $\abs{I_n^+}, \abs{I_n^-} \to \infty$ and $\frac{\abs{I_n^+}}{n},\frac{\abs{I_n^-}}{n} \to \frac{1}{2}$ a.s. Further,
% \begin{align*}
%     \frac{1}{\abs{I_n^+}} \sum_{i \in I_n^+} \exp(\vx^T \mW \vz_i), \frac{1}{\abs{I_n^-}} \sum_{i \in I_n^-} \exp(\vx^T \mW \vz_i) \to \bE[\exp(\vx^T\mW \vz_1)])~{\rm a.s.},
% \end{align*}
% and so we get by continuity, $y_n^{\rm SA}(\vx,\{\vx_i\}_1^n,\{y_i\}_1^n;\mW) \to \tanh(\vx^T\mW \vh)  = y^{\rm CME}(\vx,\vh; \mW)$ a.s.

% % For $n$ \emph{large}, this is the optimal thing to do. But, what happens when $n$ is small? The transformer might do some bias variance kind of trade off to fit $\mW$.

% We ask the following questions:
% \begin{enumerate}[label=(\roman*)]
%     \item With the intuition that $y^{\rm CME}$ is the best estimate given $\vh$, and plugging $\mW = \bSigma^{-1}$ a softmax attention layer would implement it, is $\mW^* = \bSigma^{-1}$ the global minimizer of $\cL$?
%     \item If we start we arbitrary $\mW^0$ as perform gradient descent in the large context limit ($N$ large), then can we guarantee $\mW^{k} \to \bSigma^{-1}$ as $k\to \infty$?
%     \item What happens when there are two types of noise in the training data $\vz^{(1)} \sim \cN(\0, \bSigma_1)$ and $\vz^{(2)}\sim \cN(\0, \bSigma_2)$?
% \end{enumerate}



% \subsection{Global minimizer of the asymptotic loss}

% In this section, we answer (i) in the affirmative. Denote $\cL_n(\mW) \triangleq \bE[(y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)-y)^2]$, and consider the loss in the limit as $n\to\infty$ defined as $\cL(\mW) \triangleq \limsup_{n\to \infty} \cL_n(\mW)$. We want to show that $\mW^* = \bSigma^{-1}$ is the minimizer of $\cL$.

% We know from the previous section that $\lim_{n\to \infty} y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW) = y^{\rm CME}(\mW)$ a.s. Now, since
% \begin{align*}
%     \abs{y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)} &= \Big| \frac{\sum_{i=1}^n y_i \exp(\vx^T \mW \vx_i)}{\exp(\vx^T \mW \vx) + \sum_{i=1}^n \exp(\vx^T \mW \vx_i)} \Big| \le \frac{\sum_{i=1}^n \abs{y_i} \exp(\vx^T \mW \vx_i)}{\sum_{i=1}^n \exp(\vx^T \mW \vx_i)} = 1,
% \end{align*}
% we have that $\forall \mW \in \bR^{d\times d}, \forall n\ge 0$, $0\le g_n(\mW) \triangleq (y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW)-y)^2 \le 4$. Therefore, $\{g_n(\mW)\}_1^\infty$ are bounded, integrable random variables. Thus, using the bounded convergence theorem, we get
% \begin{align*}
%     \cL(\mW) \triangleq \limsup_{n\to \infty}\bE[g_n(\mW)] = \bE[\limsup_{n\to\infty} g_n(\mW)] &= \bE[(\limsup_{n\to\infty}y_n^{\rm SA}(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n; \mW) -y)^2] \\
%     &=\bE[(y^{\rm CME}(\mW)-y)^2] \triangleq \delta(\mW).
% \end{align*}

% Consider the problem $\min_{\hat{y}_n \in \cY_n} \bE[(\hat{y}_n-y)^2]$, where $\cY_n \triangleq \{f \in L^2: f ~{\rm is}~\sigma(\vx, \{\vx_i\}_1^n, \{y_i\}_1^n, \vh){\rm-measurable}\}$. Then, the minimizer is the conditional expectation given by
% \begin{align*}
%     \hat{y}^*(\vx, \{\vx_i\}_1^{n}, \{y_i\}_1^n, \vh) &= \bE[y \mid \vx, \{\vx_i\}_1^{n}, \{y_i\}_1^n, \vh] = \bE[y \mid \vx, \vh] = \tanh(\vx^T \bSigma^{-1}\vh) \triangleq y^{\rm CME}(\bSigma^{-1}),
% \end{align*}
% and the minimum value is $\bE[(y^{\rm CME}(\bSigma^{-1})-y)^2] = \delta(\bSigma^{-1})$. 
% Thus, we just showed that $\forall n \ge 0,\forall \hat{y}_n \in \cY_n$, we have $\bE[(\hat{y}_n-y)^2] \ge \delta(\bSigma^{-1})$. In particular, $\forall \mW \in \bR^{d\times d}$, $\forall n \ge 0$ since $y_n^{\rm SA}(\cdot ;\mW) \in \cY_n$, we have $\cL_n(\mW) \ge \delta(\bSigma^{-1})$. Therefore, for any $\mW \in \bR^{d\times d}$, we get $\cL(\mW) = \limsup_{n\to \infty} \cL_n(\mW) \ge \delta(\bSigma^{-1}) = \cL(\bSigma^{-1})$, whence $\mW^* \triangleq \bSigma^{-1}$ is the global minimizer of $\cL$.

% \subsection{Convergence of the gradient descent}


% In this section, we \emph{try} to show that (ii) is true (not much of a success). Let $\mu$ be the distribution of $\vh$. From the previous section, we have that
% \begin{align*}
%     \cL(\mW) = \delta(\mW) &= \bE[(\tanh(\vx^T \mW \vh)-y)^2] \\
%     &= \bE_{y, \vh, \vz}[(\tanh((y\vh^T+\vz^T)\mW \vh)-y)^2].
% \end{align*}
% We have that 
% \begin{align*}
%     \phi_\vh(y) &\triangleq \bE_{\vz}[(\tanh((y\vh^T+\vz^T)\mW \vh)-y)^2] \\
%     &= \bE_{\vz}[(-\tanh((-y\vh^T-\vz^T)\mW \vh)-y)^2] \\
%     &= \bE_{\vz}[(\tanh((-y\vh^T-\vz^T)\mW \vh)-(-y))^2] \\
%     &= \bE_{\tilde{\vz} \triangleq -\vz}[(\tanh((-y\vh^T+\tilde{\vz}^T)\mW \vh)-(-y))^2] \\
%     &= \bE_{\vz}[(\tanh(((-y)\vh^T+\vz^T)\mW \vh)-(-y))^2] = \phi_\vh(-y).
% \end{align*}
% Thus, we get
% \begin{align*}
%     \cL_\mu(\mW) = \bE_{y, \vh\sim \mu}[\phi_\vh(y)] = P(y=1)\bE_\vh [\phi_\vh(1)]+P(y=-1)\bE_\vh [\phi_\vh(-1)] = \frac{1}{2} \bE_{\vh}[\phi_\vh(1) + \phi_\vh(-1)] = \bE_\vh[\phi_\vh(1)],
% \end{align*}
% and so, $\cL_\mu(\mW) = \bE_{\vh\sim \mu,\vz \sim \cN(\0, \bSigma)}[(\tanh((\vh^T+\vz^T)\mW\vh)-1)^2]$. Notice that although the minimizer $\mW^* = \bSigma^{-1}$ of $\cL$ is independent of the distribution $\mu$ of $\vh$, the minimum value $\cL_\mu(\bSigma^{-1})$ depends on $\mu$. Noting that $1-\tanh(z) = 1 - \frac{1-e^{-2z}}{1+e^{-2z}} = \frac{2e^{-2z}}{1+e^{-2z}} = \frac{2}{1+e^{2z}}$, we can write $\cL_\mu(\mW; \bSigma) = \bE_{\vh\sim \mu}[\psi_\vh(\mW; \bSigma)]$, where
% \begin{align*}
%     \psi_\vh(\mW; \bSigma) \triangleq \bE_{\vz\sim\cN(\0, \bSigma)}[(1-\tanh((\vh^T+\vz^T)\mW\vh))^2]= 4\bE_{\vz\sim \cN(\0,\bSigma)}\Big[\frac{1}{(1+\exp(2(\vh^T+\vz^T)\mW\vh))^2}\Big].
% \end{align*}
% The result from the previous section is that for any $\0 \prec \bSigma \in\bR^{d\times d}, \vh\in \bR^d$, we have $\psi_\vh(\mW; \bSigma) \ge \psi_\vh(\bSigma^{-1}; \bSigma)$ for all $\mW \in \bR^{d\times d}$.

% \subsubsection{Detour to verify the above claim}
% Let $d = 1, \bSigma = \sigma^2 > 0, \mW = \omega$. Then, we have that $\psi_h(\omega;\sigma^2) \ge \psi_h(\sigma^{-2}; \sigma^2)$ for any $\omega \in \bR$.
% \begin{align*}
%     \psi_h(\omega; \sigma^2) &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{\exp(-z^2/2\sigma^2)}{(1+\exp(2\omega h(h+z)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp(z^2/\sigma^2)+\exp(z^2/\sigma^2+2\omega h(h+z)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp((z/\sigma)^2)+\exp((z/\sigma)^2+2(\omega\sigma h)(z/\sigma) + \omega^2\sigma^2h^2+(2\omega h^2-\omega^2\sigma^2 h^2)))^2} dz \\
%     &= \frac{4}{\sqrt{2\pi \sigma^2}} \int_{z=-\infty}^\infty \frac{1}{(\exp((z/\sigma)^2)+\exp(h^2(2\omega-\omega^2\sigma^2))\exp((z/\sigma + \omega \sigma h)^2))^2} dz .
% \end{align*}
% The intuition is that we wish to maximize $\kappa(\omega;\sigma^2) \triangleq 2\omega-\omega^2\sigma^2$ in the denominator in order to minimize the above function, which happens at $\omega^* = \sigma^{-2}$.

% Clearly $\kappa$ is concave in $\omega$. Does this imply that $\psi_h(\omega; \sigma^2)$ is convex in $\omega$?

% \subsection{Effect of the covariance}
% If $\vh \sim \cN(\0, \bSigma)$, and $\vh$ is known (or in the regime of obtaining a good estimate of it, for example large $N$), then the optimal estimate of $y$ from $\vx = \vh y + \vz$, $\vz \sim \cN (\0, \sigma^2\mI_d)$ is $\hat{y} = \frac{\vh^T \vx}{\norm{\vh}_2^2 + \sigma^2}$



% We aim to show that when $N$ is large $\mW = \alpha \mI_d$ for some $\alpha \ge 0$ large.





==> contents/transformers-for-ICE.tex <==
\section{Experiments with Multi-Layer Transformers}
\label{in_context_estimation}
In this section, we provide a comprehensive overview of our experiments with multi-layer transformers, detailing the experimental setup, training methodologies, and the relevant baselines for each scenario.
% Consider a more general class of in-context estimation problems than Problem \ref{def:ice-subclass}. Estimate $\vx_t \in \cX \subset \bR^{d_\vx}$ from the observations $\vy_t \in \bR^{d_\vy}$, where $\vy_t = f(\vx_t, \vh_t(\theta), \vz_t)$, i.e., the observation $\vy_t$ is a function of $\vx_t$, a latent context dependent parameter $\vh_t(\theta) \in\bR^d$, and an independent noise $\vz_t \in \bR^{d_z}$, for $t \in [n] \triangleq \{1, \dots, n\}$. Here, $n$ denotes maximum context length. We assume that the random processes are generated as $\{\vx_t\}_{t\in[n]} \sim P_x, \{\vz_t\}_{t\in[n]} \sim P_z, \{\vh_{t}\}_{t\in[n]} \sim P_{h\mid\theta}$, where distribution $P_{h\mid \theta}$ is determined by a latent parameter $\theta$. The latent parameter is drawn from a distribution $P_\Theta$ on the latent space $\Theta$. We assume that the random processes $\{\vx_t\}_{t\in[n]}$ and $\{\vh_t(\theta)\}_{t\in[n]}$ are independent from each other for all $\theta \in \Theta$. Denote $\cP^k_\theta = \{(\vy_t, \vx_t), t\in[k]\}$ to be the set of example prompts until time $k$.

% Consider the general problem as in Definition \ref{def:ice}.


% Given the past $k$ examples $\cP_\theta^k$ from the context $\theta\in \Theta$ and the current observation $\vy_{k+1}$, the context unaware (CU) minimum mean squared error estimate (MMSE) of $\vx_{k+1}$ is known to be the conditional expectation
% \begin{equation}
% \label{eq:context_agnostic_estimator}
%     \hat{\vx}_{k+1}^{\rm CU}(\cP_\theta^k, \vy_{k+1}) = \bE_{\vx \sim \bP_x}[ \vx_{k+1} = \vx \mid \cP_\theta^k, \vy_{k+1}].
% \end{equation}

% In addition, if the estimator knows the latent context parameter $\theta$ apriori, then the context aware (CA) optimal estimator is given by
% \begin{equation}
% \label{eq:in_context_estimator}
%     \hat{\vx}_{k+1}^{\rm CA}(\cP_\theta^k, \vy_{k+1};\theta) = \bE_{\vx \sim \bP_x}[ \vx_{k+1} = \vx \mid \cP_\theta^k, \vy_{k+1}, \theta],
% \end{equation}
% which we call the optimal context-aware estimator. It is known that the MSE achieved by an optimal context-aware estimator not worse than that of a context agnostic estimator given by Equation \ref{eq:context_agnostic_estimator}.

% Having a closer look at the computation of the conditional expectation in \ref{eq:context_agnostic_estimator}, we get
% \begin{align*}
%     &\hat{\vx}_{k+1}^{\rm CU}(\cP_\theta^k, \vy_{k+1}) = \bE[ \vx_{k+1} = \vx \mid \cP_\theta^k, \vy_{k+1}] = \sum_{\vx \in \cX} \vx \bP_x(\vx_{k+1} =  \vx \mid\cP_\theta^k, \vy_{k+1}) \\
%     &\hspace{20pt} \propto \sum_{\vx\in \cX} \vx \bP_x(\vx) p(\cP_\theta^k, \vy_{k+1} \mid \vx) \\
%     &\hspace{20pt} =\sum_{\vx\in \cX}\vx \bP_x(\vx) \int_{\theta' \in \Theta} p_\Theta(\theta')\int_{\mH_1, \dots, \mH_k, \mH_{k+1} \in \bR^{d_{\vy}\times d_{\vx}}} p_{h \mid \theta'}(\mH_1, \dots, \mH_k, \mH_{k+1}) \\
%     &\hspace{50pt} p(\cP_\theta^k, \vy_{k+1} \mid \vx, \mH_{1}, \dots, \mH_k, \mH_{k+1})~ d\mH_1 \dots d\mH_{k+1},
% \end{align*}
% The above computation involves evaluating a multi-dimensional integral. In most practical problems of estimation, computation of \ref{eq:context_agnostic_estimator} can be very difficult or even intractable. We train a transformer and demonstrate its effectiveness in approximating Equation \ref{eq:context_agnostic_estimator}.

% This is indeed the case with the wireless communication problem of interest (see Section. \ref{wireless_communication_problem}). Motivated by recent studies (\cite{garg2023transformers}) that demonstrate the remarkable ability of transformers to exhibit in-context learning, we train a transformer-based model to approximate \ref{eq:context_agnostic_estimator}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Multi-layer transformers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure below %%%%%%%%%%%%%
\begin{figure}[ht]
\centering
\input{figures/TransformerModel}
\caption{Transformer model performing causal attention}
\label{fig:TransformerModel}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure above %%%%%%%%%%%%%

% Let $\mT(\cdot; \{\mW^\ell\}_1^L)$ denote a decoder-only transformer \cite{gpt2} with parameters (weights) $\{\mW^\ell\}_1^L$, where the $\ell$th layer contains $\mW^\ell \equiv (\{\mW^\ell_{Q,h}, \mW_{K,h}^\ell, \mW_{V,h}^\ell\}_{h=1}^H, \mW^\ell_{\rm MLP})$. Let $\mT_{k}(\cP_{k}, \vy_{k+1}) \in \bR^{d_\vx}$ be estimated value of $\vx_{k+1}$ by the transformer given $\cP_k, \vy_{k+1}$ (see Fig. \ref{fig:TransformerModel}). Denote the data set $\mathcal{D}=\{ \cP_n^b = \{(\vy_t^b, \vx_t^b)\}_{t=1}^n \mid {\rm for~each}~b\in [B],  \theta \sim P_{\Theta}, \vx_k \sim P_\cX, \vz_k \sim P_z, \vh_k(\theta) \sim P_{h \mid \theta}, \vy_k = f(\vx_k, \vh_k(\theta), \vz_k)\}$ of trajectories generated via our sampling procedure. We first sample $\theta \sim P_{\Theta}, \{\vx_k\} \sim P_\cX,$ and $\{\vz_k\} \sim P_z$ independent of each other. We then sample $\{\vh_t(\theta)\} \sim P_{h \mid \theta}$ using $\theta$ and use the sampled quantities to compute $\vy_k = f(\vx_k, \vh_k(\theta), \vz_k)$. We repeat this to sample $N$ batches of size $B$ of maximum context length $n$.

% Then, we can train the transformer by minimizing the sum of the squared norms of the difference between the predicted value and the actual values, i.e., we optimize $\{\mW^i\}_1^\ell$ such that the loss defined below is minimized:
% \begin{align}
% \label{eq:loss_function}
%      \mathcal{L}(\{\mW^\ell\}_1^L; \mathcal{D}) &= \frac{1}{N B} \sum_{b=1}^{NB} \sum_{k=0}^{n-1} \norm{\mT_{k}(\cP_{k}^b, \vy_{k+1}^b; \{\mW^\ell\}_1^L) - \vx_{k+1}^n}_2^2 \\
%      &\approx \sum_{k=1}^{n-1}\bE[\norm{\mT_k(\cP_{k}, \vy_{k+1}; \{\mW^\ell\}_1^L) - \vx_{k+1}}_2^2] \nonumber.
% \end{align}

% Let $\mT_k(\cdot; \{(\mW^*)^\ell\}_1^L)$ denote the \emph{trained} transformer. In the setting of in-context estimation, we are interested in the performance of $\mT_k(\cP_k, \vy_{k+1}; \{(\mW^*)^\ell\}_1^L)$ as a function of $k$.



\subsection{Experimental setup}

We study the performance of multi-layer transformers empirically through the following experimental setup, which is inspired by common communication systems.
We choose the input space to be $\tilde{\cX} \triangleq \{\pm 1 \pm i: i\triangleq \sqrt{-1}\}$, which is a finite subset of the circle of radius $\sqrt{2}$ in $\bC$.
We assume that these symbols are equally likely, $\bP_x \equiv \cU(\tilde{\cX})$.
The noise is distributed as $\bP_z \equiv \cC\cN(\0, 2\sigma^2 \mI_d)$. The quantity $1/\sigma^2$ is called the signal-to-noise ratio (SNR).

We consider two scenarios depending on the nature of the hidden parameter process $\tilde{\vh}_t(\theta)$.


\subsubsection{Scenario 1: Time invariant process}

The setup is similar to that of our theoretical results. The hidden context $\theta$ can be either $0$ or $1$, i.e., $\Theta \triangleq \{0,1\}$. We consider $\bP_\Theta = \cU(\Theta)$, the uniform distribution on $\Theta$. The distributions $\bP_{h \mid \theta}$ is described next for $\theta \in \Theta$.
For $\theta = 0$, the $j$th component of $\tilde{\vh}(0)$ is given as 
\begin{align*}
   \tilde{h}^j(0) = \exp \left( \frac{-i\pi(j-1)\cos(\alpha)}{2} \right) \triangleq  \tilde{h}^j_\alpha(0), \quad j\in [d], \quad \alpha \sim \cU((0, \pi]),
\end{align*}
where the subscript denotes the dependence on $\alpha$. The above distribution corresponds to a one-ray line-of-sight channel in wireless communication \cite{goldsmith_2005}, where $\alpha$ is the angle of arrival of the incoming signal at the receiver, and the antenna spacing is $(1/4)$th of the wavelength of the carrier.
When $\theta = 1$, we have 
\begin{align*}
    \tilde{\vh}(1) \sim \cC\cN(\0, \mI_d).
\end{align*}
This is referred to as the independent and identically distributed (i.i.d) Rayleigh fading channel model in the wireless communication literature \cite{goldsmith_2005}.


\subsubsection{Scenario 2: Time varying process}

Let latent space $\Theta$ be a compact subset of $\bR_+$, and let $\bP_{\Theta} = \cU(\Theta)$ be the uniform distribution over $\Theta$.
Further, assume $\{h^j_t(\theta)\}_{t\ge 1}$ are iid zero-mean wide-sense stationary (WSS) Gaussian processes (Section 15.5, \cite{Kay97}) across $j\in[d]$ with
\begin{equation}
\label{eq:scenario-2-h-dist}
    \bE \left[ h^j_t(\theta) h^j_{t+k}(\theta) \right] \triangleq R_\theta(k)
    = J_0 \left( \frac{2\pi f_{c} T_s k \theta}{c} \right), \quad k\ge 0
\end{equation}
where $J_0 (\cdot)$ is the Bessel function of the first kind of order zero. The above distribution is referred to as Clarke's model (Section 3.2.1, \cite{goldsmith_2005}) for time varying channel processes in wireless communication. The constants $T_s, f_c, c$ denote the carrier frequency, symbol duration, and the velocity of light respectively. The latent context $\theta$ denotes the relative velocity between the transmitter and the receiver.

\subsection{Training}
\label{sec:training}

We adopt the training setup described in \cite{panwar2024incontext}, which is in turn based on the approach used in \cite{garg2023transformers} with minor changes to account for complex-valued symbols. 
For all experiments, we train a GPT-2 \cite{radford2019language} decoder-only model from scratch.
As shown in \ref{fig:TransformerModel}, we train our decoder models to perform prediction in the style of language models, where $$((\vy_1, \vx_1), (\vy_2, \vx_2), \dots, (\vy_n, \vx_n), \vy_{n+1})$$ are used to predict $\vx_{n+1}$. The vectors $\vx_t$ are appended with $(2d-2)$ zeros to have the same dimension as $\vy_t\in \bR^{2d}$. We remark that the construction of the prompt in this way is different from that in our theoretical results, where $\vy_t, \vx_t$ are concatenated into a single token. We use the sum of squared errors between all $(\vx_t, \hat{\vx}_t), t\in[n+1]$ as our loss function, where $\hat{\vx}_t$ is the estimate of the transformer for $\vx_t$. This is also different from that in our theoretical results where the loss is only on the last token. To generate a mini-batch of prompts, first we sample $\theta \sim \bP_\Theta$, and then we independently sample $\{\tilde{\vh}_t(\theta)\}_{t\in[n+1]}$ for each of the prompts in the mini-batch. 



% The training data is generated as follows. First we draw $\theta \sim {\rm Unif}(\Theta)$. In C1, we generate $\alpha \sim {\rm Unif}[0, \pi)$ and set $h^j_t(0) = \phi_j(\alpha)$. In C2, we generate the sequence $\vh^j = (h_t^j, t\in \bN)$ from a stationary Gaussian random process. For each training mini-batch, we re-sample $\theta$ and then independently sample each $\vh^j$.

% As done in \cite{ahuja2023incontext}, we train our decoder models to perform prediction in the style of language models, where $$((\vy_1, \vx_1), (\vy_2, \vx_2), \dots, (\vy_k, \vx_k), \vy_{k+1})$$ are used to predict $\vx_{k+1}$. We use the sum of squared errors between all $(\vx_t, \hat{\vx}_t), t\in[k+1]$ as our loss function, where $\hat{\vx}_t =  T_W^{k+1}(S_k, \vy_{k+1})$. 

In all the experiments, we set $d = 4$, and the constants $f_c = 2.9\times 10^9~{\rm Hz}, T_s = 1~{\rm ms}, c = 3\times 10^8~{\rm m/s}$. For scenario 2, we consider $\Theta = \{5, 15, 30\}$. These are representative of the typical values seen in practice for wireless communications. 

We include our model architecture details and other hyper-parameter settings in Appendix~\ref{parameters}.


% The training objective is also different in the sense that the loss is the sum of all the loss values for predicted symbol $\hat{\vx}_{k+1}$ given $k$ examples and $\vy_{k+1}$ for $k\in[n]$.

% Let $\mT(\cdot; \{\mW^\ell\}_1^L)$ denote a decoder-only transformer \cite{gpt2} with parameters (weights) $\{\mW^\ell\}_1^L$, where the $\ell$th layer contains $\mW^\ell \equiv (\{\mW^\ell_{Q,h}, \mW_{K,h}^\ell, \mW_{V,h}^\ell\}_{h=1}^H, \mW^\ell_{\rm MLP})$. Let $\mT_{k}(\cP_{k}, \vy_{k+1}) \in \bR^{d_\vx}$ be estimated value of $\vx_{k+1}$ by the transformer given $\cP_k, \vy_{k+1}$ (see Fig. \ref{fig:TransformerModel}). Denote the data set $\mathcal{D}=\{ \cP_n^b = \{(\vy_t^b, \vx_t^b)\}_{t=1}^n \mid {\rm for~each}~b\in [B],  \theta \sim P_{\Theta}, \vx_k \sim P_\cX, \vz_k \sim P_z, \vh_k(\theta) \sim P_{h \mid \theta}, \vy_k = f(\vx_k, \vh_k(\theta), \vz_k)\}$ of trajectories generated via our sampling procedure. We first sample $\theta \sim P_{\Theta}, \{\vx_k\} \sim P_\cX,$ and $\{\vz_k\} \sim P_z$ independent of each other. We then sample $\{\vh_t(\theta)\} \sim P_{h \mid \theta}$ using $\theta$ and use the sampled quantities to compute $\vy_k = f(\vx_k, \vh_k(\theta), \vz_k)$. We repeat this to sample $N$ batches of size $B$ of maximum context length $n$.

% Then, we can train the transformer by minimizing the sum of the squared norms of the difference between the predicted value and the actual values, i.e., we optimize $\{\mW^i\}_1^\ell$ such that the loss defined below is minimized:
% \begin{align}
% \label{eq:loss_function}
%      \mathcal{L}(\{\mW^\ell\}_1^L; \mathcal{D}) &= \frac{1}{N B} \sum_{b=1}^{NB} \sum_{k=0}^{n-1} \norm{\mT_{k}(\cP_{k}^b, \vy_{k+1}^b; \{\mW^\ell\}_1^L) - \vx_{k+1}^n}_2^2 \\
%      &\approx \sum_{k=1}^{n-1}\bE[\norm{\mT_k(\cP_{k}, \vy_{k+1}; \{\mW^\ell\}_1^L) - \vx_{k+1}}_2^2] \nonumber.
% \end{align}

% Let $\mT_k(\cdot; \{(\mW^*)^\ell\}_1^L)$ denote the \emph{trained} transformer. In the setting of in-context estimation, we are interested in the performance of $\mT_k(\cP_k, \vy_{k+1}; \{(\mW^*)^\ell\}_1^L)$ as a function of $k$.

\subsection{Baselines}
\label{baseline_genie_descriptions}


% Already included.

% For scenario 1, we have $\hat{\vx}_{k+1}^{\rm CU-H-LMMSE}$ (context unaware) and $\hat{\vx}_{k+1}^{\rm CA-X-MMSE}$  for $\theta = 0$ and $\hat{\vx}_{k+1}^{\rm CA-H-MMSE}$ for $\theta=1$.

% For scenario 2, we have $\hat{\vx}_{k+1}^{\rm CU-H-LMMSE}$ and $\hat{\vx}_{k+1}^{\rm CA-H-MMSE}$ for all $\theta\in \Theta$.


% Computed later.

% For scenario 2, we have $\hat{\vx}_{k+1}^{\rm CU-H-MMSE}$ and $\hat{\vx}_{k+1}^{\rm CU-X-MMSE}$.

% To do.

% For scenario 2, need $\hat{\vx}_{k+1}^{\rm CA-X-MMSE}$ for all $\theta\in \Theta$.
% For scenario 1, need $\hat{\vx}_{k+1}^{\rm CA-X-MMSE}$ for $\theta=1$, and $\hat{\vx}_{k+1}^{\rm CU-X-MMSE}, \hat{\vx}_{k+1}^{\rm CU-H-MMSE}$.



In this section, we describe some feasible context-aware estimators that achieve a low MSE, along with some context-unaware estimators for both scenarios, are motivated from the wireless communications.

%$\hat{\vx}^{\rm CA/CME, \theta}$
%$\hat{\vx}^{\rm CU/CME/LMMSE}$

For scenario 1, we provide a context-aware baseline that performs the conditional mean estimate (CME) on the symbol given the context (${\rm CME}[x \mid \theta]$) (see \eqref{eq:scenario-1-aware} in Appendix). We also provide a context-unaware baseline that performs a Linear Minimum Mean Square Estimate (LMMSE) of the hidden parameter $\tilde{\vh}(\theta)$, and uses this estimate to perform a CME on x (denoted as ${\rm CME}[x \mid {\rm MMSE}[h]]$) (see Appendix \ref{appen:typical-baselines}). Both these baselines require the knowledge of the statistics of the hidden parameter $\tilde{\vh}(\theta)$.

%or $\hat{\vx}^{\rm CA/CME/MMSE}$
%or $\hat{\vx}^{\rm CU/CME/MMSE}$
%or $\hat{\vx}^{\rm CU/CME}$

For scenario 2, we provide four baselines, a context-aware baseline and three context unaware baselines. The context-aware baseline first performs a Minimum Mean Squared Error (MMSE) estimate on the hidden parameter process ${\tilde{\vh}_t}$ given $\theta$, and uses this MMSE estimate to compute the CME on the symbol given the context (${\rm CME}[x\mid{\rm MMSE}[h\mid\theta]]$). The first context-unaware baseline is ${\rm CME}[x \mid {\rm LMMSE}[h]]$ which is similar to the one in scenario 1, albeit as the distributions are different in each scenario the computation of the quantities would vastly differ. The second context-aware estimate computes an MMSE on ${\tilde{\vh}_t}$ (without any knowledge of $\theta$) and uses this estimate to perform CME on the symbol (${\rm CME}[x \mid {\rm MMSE}[h]]$ ). The last context-aware baseline we provide computes a direct CME on the symbol (${\rm CME}[x]$) (without any knowledge of $\theta$). These additional baselines were included to gain better insights into understanding which baseline the transformer closely matches in this harder scenario. Further details about the computation of the baselines are provided in Appendix \ref{appen:baselines}.



% when $\theta = 0$,  the randomness of the hidden parameter $\tilde{\vh}(0)$ comes from a single scalar random variable $\alpha$, due to which the computation of the posterior mean requires an integral in one dimension.
% It can therefore be calculated in a computationally efficient manner. The exact expression appears in \ref{eq:one_ray_model_symbol_estimation}. 
% In the remaining cases, we cannot evaluate the expression explicitly. In these cases, the context-aware estimator first computes the Linear Minimum Mean Square Estimate (LMMSE) $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$  of the channel parameter ${\vh}_{k+1}(\theta)$ given $\cP_\theta^k$ and $\theta$. The exact details of computing the expression for $\hat{\vh}_{k+1}^{\rm LMMSE, \theta}$ are given in Appendix \ref{context_aware_estimators_derivation}. Incidentally, for all these cases, since $\vh_{k+1}(\theta)$ and $(\vy_t, t\in [k])$ are jointly Gaussian, conditioned on $(\vx_t, t\in[k])$, this channel estimate is the minimum mean squared estimate (MMSE) of $\vh_{k+1}(\theta)$ given $\cP_\theta^k, \theta$. Then, the symbol is estimated by computing $\bE[\vx_{k+1} \mid \vh_{k+1}(\theta) = \hat{\vh}_{k+1}^{\rm MMSE, \theta}, \vy_{k+1}]$; the exact expression for above conditional expectation is given in \eqref{eq:symbol_estimate}.

% For the context-unaware baseline, we describe an estimation procedure commonly used in wireless communication. The estimator first computes the LMMSE of the channel (see Appendix \ref{baseline_for_agnostic_estimators}), which uses the correlation matrices corresponding to the prior for the channel parameter process. Then, it estimates the symbol as the conditional mean, conditioned on the LMMSE for the channel. The exact details are given in Appendix \ref{appen:baselines}.








==> contents/wireless-communication-model.tex <==

\section{Wireless Communication System Model}
\label{wireless_communication_problem}

In this section, we specialize the estimation problem stated in Section \ref{in_context_estimation} to the wireless communication problems of interest.
Consider a wireless channel with a single transmit antenna and $d$ receive antennae (see Fig. \ref{fig:TranEstimator}). Let $s_t \in \cX = \{x_I+ \sqrt{-1} \ x_Q  \mid x_I, x_Q\in\{\pm 1\}\}$ be the $t$th transmitted symbol.
The transmit sequence $\{s_t\}$ is an i.i.d sequence of symbols drawn from $\cX$ with uniform probability.

Let $\vy_t \in \bC^d$ be the received symbol vector, where $y^j_t$ denotes the received symbol at the $j$th antenna at time $t$. 
Let $\vh_t(\theta) \in\bC^d$ be the wireless channel coefficient between the transmitter and the $j$th receiver antenna, and let $\vz_t$ be the additive noise at the receiver, at time $t$. 
Then, we can write the input-output relation as
\begin{equation}
\label{eq:io_relation}
    \vy_t = \vh_t(\theta) s_t + \vz_t, \quad t\in[\ell].
\end{equation}



%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure below %%%%%%%%%%%%%
\begin{figure}[ht]
\centering
\input{figures/TranEstimator}
\caption{Notional diagram of a typical single-input multiple-output (SIMO) wireless channel combined with a transformer-based receiver}
\label{fig:TranEstimator}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% main figure above %%%%%%%%%%%%%

For some $\sigma^2 > 0$, the sequence $\{\vz_t\}$ are independent and identically distributed (i.i.d.) Gaussian random vectors, with $\vz_{t, I},\vz_{t,Q}\sim \mathcal{N}(\mathbf{0}, \sigma^2 \mI_{d})$ for each $t\in[\ell]$. The ratio $1/\sigma^2$ is called the signal-to-noise-ratio (SNR).




Next, we describe the latent context space $\Theta$, and the conditional distributions for the channel, i.e., $P_{h\mid \theta}$ for $\theta\in\Theta$. The channel parameter process $\{\vh_t(\theta)\}$ in the wireless communications typically depends on two aspects, discussed in the following subsections.


\subsection{Type of Scattering}

In wireless communication, signals transmitted from the transmitter antenna reach the receiver antenna from multiple directions after being scattered by the obstacles in the environment. In this situation, the channel parameter depends on the configuration of the environment and the positioning and influence of the obstacles. If there are few or no obstacles, there is a direct path called the line-of-sight (LoS) path between the transmitter and the receiver, and in this case, the received signal can be modeled by a single ray of signal reaching the antenna. Thus, the effective channel parameter depends on the angle of arrival of this LoS component of the signal. On the other hand, if there are significantly many scatterers in the environment, as in an urban environment, there is a large number of reflected rays reaching the receiver at the same time. This scenario is (aptly) called the rich-scattering environment, and the channel parameter in this case can be approximated as a Gaussian random variable. 

Each of the above cases gives rise to a different distribution on the channel, and hence, we model the type of scattering of the signal as the latent context $\theta$. More formally, let $\Theta=\{0, 1\}$ denote the latent context space where $\theta = 0$ corresponds to the LoS model, and $\theta=1$ corresponds to the rich scattering model. In this case, we first generate $\vh_1(\theta)$ and assume that it remains constant for the period of interest, i.e., $\vh_t(\theta) = \vh_1(\theta)$ for all $t\in[\ell]$. This corresponds to the environment being stationary, i.e., the signal paths do not change over time in the period of interest.

    When $\theta=0$, $h_1^j(0) = \exp(-(\sqrt{-1})2\pi (s/\lambda)(j-1)\cos(\alpha)) \triangleq \phi_j(\alpha)$, where $j\in[d]$. 
    
    Here, $\alpha \sim {\rm Unif}[0, \pi)$ is the angle of arrival of the one ray (\cite{goldsmith_2005}), $s$ is the spacing between the antennae, $\lambda$ is the wavelength of the signal used for transmission.

    When $\theta=1$, the channel parameter is modeled by $\vh_{1, I}(1),\vh_{1, Q}(1) \sim \mathcal{N}(0, \frac{1}{2}\mI_d)$, with $\vh_{1, I}(1), \vh_{1, Q}(1)$ are drawn independently. We call the above case as scenario C1.

\subsection{Mobility}

Assume that the transmitter is fixed and the receiver is moving towards the transmitter with some velocity $v$ m/s. This situation naturally arises in the wireless communication application. Considering a rich-scattering environment, the properties of the channel parameter, and the correlation of the parameter process depends on the velocity: more the velocity, less the correlation. Therefore, having a estimate of the velocity in such environments and the correlation structure would greatly improve the performance of the estimator at the receiver. However, in practice, this can be difficult to obtain online. Hence, we model velocity to parameterize the latent context $\theta$. 

More specifically, we consider a latent space $\Theta = [M]$  representing the $M$ possible velocities with $v_\theta$ being the mobile velocity when the latent variable is $\theta$. Let $\{h^j_t(\theta)\}_t$ denote the channel parameter process at the $j$th antenna. Note that this process is a time-varying process with unlike in the last scenario, where the process that remains constant across the time. Across the antennae $j\in[d]$, we assume that the processes $\{h^j_t(\theta)\}_t$ are  i.i.d. zero-mean, wide-sense stationary Gaussian random processes (Section 15.5, \cite{Kay97}). The correlation function $R_\theta(m) = \bE[h_{t, I}^1(\theta) h^1_{m+t, I}(\theta)]$ for any $t\in\bN$ is determined by the latent context $\theta$. We use the well-known Clarke's model (Section 3.2.1, \cite{goldsmith_2005})and set $R_\theta(m) = J_0(\frac{2\pi T_s m v_\theta}{\lambda})$. Here, $T_s$ is the symbol duration, $\lambda$ is the wavelength of the signal, $v_\theta$ is the relative velocity between the transmitter and the receiver, $J_0$ denotes the Bessel function of the first kind of order $0$. 
We call the above scenario as scenario C2.


In both the scenarios C1 and C2, the latent parameter $\theta$ is drawn uniformly at random from $\Theta$. 


In wireless communications, a set of known symbols called pilots are transmitted as part of the transmitted symbols. 
These symbols are used to estimate the channel parameter process and then the estimate is typically used to perform symbol estimation. 
There is a natural way in which these pilots can be used as in-context examples. 
In the language of Section \ref{in_context_estimation}, the set $S_k$ contains the pilots symbols $(s_t, t\in[k])$ until time $k$
and the corresponding received symbols $(\vy_t, t\in[k])$. 
The pilots do not communicate any information and hence, it is important to keep the number of pilots small. 
Thus, machine learning model based estimators need to be information-efficient and make maximal use of the information in $S_k$.


==> figures/TranEstimator.tex <==
\begin{tikzpicture}
  [
  font=\small, line width=1pt,
  check/.style={rectangle, minimum height=2.5mm, minimum width=2.5mm, draw=black},
  varnode/.style={circle, minimum size=2mm, draw=black},
  mmse/.style={rectangle, minimum height=7.5mm, minimum width=25mm, rounded corners, draw=black},
  quantity/.style={rectangle, minimum height=8mm, minimum width=8mm, rounded corners, draw=black},
  multiply/.style={trapezium, trapezium angle=75, draw=black, minimum width=10mm, minimum height=8mm, rounded corners}
  ]

  \draw[draw=black, rounded corners] (2.5,-1.5) rectangle (5.5,1.5);
  \node at (4,0) {Transformer};

  \draw[->] (5.5,0) to node[above]{$\hat{s}_t$} (8,0);

  \draw[->] (1,1.375) to (1.25,1.75) to (0.75,1.75) to (1,1.375) to (1,1) to node[above]{$y_t^1$} (2.5,1);
  \draw[->] (1,0.375) to (1.25,0.75) to (0.75,0.75) to (1,0.375) to (1,0) to node[above]{$y_t^2$} (2.5,0);
  \draw[->] (1,-0.625) to (1.25,-0.25) to (0.75,-0.25) to (1,-0.625) to (1,-1) to node[above]{$y_t^d$} (2.5,-1);

  \draw[->] (-3,0) to node[above]{$s_t$} (-1.75,0);
  \draw[dashed,shorten <=5pt] (-1.75,0) -- node[above,yshift=5pt]{$h_t^1 (\theta)$} (0.75,1.5);
  \draw[dashed,shorten <=5pt] (-1.75,0) -- node[below,xshift=15pt,yshift=3pt]{$h_t^2 (\theta)$} (0.75,0.5);
  \draw[dashed,shorten <=5pt] (-1.75,0) -- node[below]{$h_t^d (\theta)$} (0.75,-0.5);

  \draw[<-,densely dotted,rounded corners] (-0.375,-1) to (-0.375,-1.625) to node[above] {Context $\theta$} (-2.25,-1.625);
\end{tikzpicture}

==> figures/TransformerModel.tex <==
% \input{preamble}
\begin{tikzpicture}
  [
  font=\small, line width=1pt,
  check/.style={rectangle, minimum height=2.5mm, minimum width=2.5mm, draw=black},
  varnode/.style={circle, minimum size=2mm, draw=black},
  mmse/.style={rectangle, minimum height=7.5mm, minimum width=25mm, rounded corners, draw=black},
  quantity/.style={rectangle, minimum height=8mm, minimum width=8mm, rounded corners, draw=black},
  multiply/.style={trapezium, trapezium angle=75, draw=black, minimum width=10mm, minimum height=8mm, rounded corners}
  ]

  \draw[draw=black, rounded corners] (2.5,-1.5) rectangle (8.5,1.5);
  % \node at (6,0) {Transformer};


\node[below] at (3.0, -2) {$\mathbf{y}_0$};
\draw[->] (3.0, -2) to (3.0, -1.5);
\node[below] at (3.5, -2) {$\mathbf{x}_{s_0}$};
\draw[->] (3.5, -2) to (3.5, -1.5);


\draw[dashed,shorten <=5pt] (3, -1.5) to (3.5, 1.5);


\node[below] at (4.0, -2) {$\mathbf{y}_1$};
\draw[->] (4.0, -2) to (4.0, -1.5);
\node[below] at (4.5, -2) {$\mathbf{x}_{s_1}$};
\draw[->] (4.5, -2) to (4.5, -1.5);

\node at (5.5, 2.0){$\dots$};
\node at (5.25, -2.0){$\dots$};



\draw[dashed,shorten <=5pt] (3, -1.5) to (4.5, 1.5);
\draw[dashed,shorten <=5pt] (3.5, -1.5) to (4.5, 1.5);
\draw[dashed,shorten <=5pt] (4, -1.5) to (4.5, 1.5);


\node[below] at (6, -2) {$\mathbf{y}_{N-1}$};
\draw[->] (6, -2) to (6, -1.5);
\node[below] at (6.5, -2) {$\mathbf{x}_{s_{N-1}}$};
\draw[->] (6.5, -2) to (6.5, -1.5);

\node[below] at (7.1, -2) {$\mathbf{y}_{N}$};
\draw[->] (7.0, -2) to (7.0, -1.5);


\draw[->] (3.5, 1.5) to node[above=7pt]{$\mT_0$} (3.5, 2.0);
\draw[->] (4.5, 1.5) to node[above=7pt]{$\mT_1$} (4.5, 2.0);
\draw[->] (7.5, 1.5) to node[above=7pt]{$\mT_{N}$} (7.5, 2.0);

\draw[dashed,shorten <=5pt] (3, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (3.5, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (4, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (4.5, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (6.0, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (6.5, -1.5) to (7.5, 1.5);
\draw[dashed,shorten <=5pt] (7.0, -1.5) to (7.5, 1.5);

\draw[<->, thick] (3, -3) to (6.5, -3);
\node at (4.5, -2.75) {$\vy_0^{N-1}, \vx_{s_0}^{N-1}$};


  % \draw[->] (5.5,0) to node[above]{Estimate of $x_t$} (8,0);

  % \draw[->] (1,1.375) to (1.25,1.75) to (0.75,1.75) to (1,1.375) to (1,1) to node[above]{$y_t^1$} (2.5,1);
  % \draw[->] (1,0.375) to (1.25,0.75) to (0.75,0.75) to (1,0.375) to (1,0) to node[above]{$y_t^2$} (2.5,0);
  % \draw[->] (1,-0.625) to (1.25,-0.25) to (0.75,-0.25) to (1,-0.625) to (1,-1) to node[above]{$y_t^d$} (2.5,-1);

  % \draw[->] (-3,0) to node[above]{$x_t$} (-1.75,0);
  % \draw[dashed,shorten <=5pt] (-1.75,0) -- node[above,xshift=5pt]{$h_t^1 (\theta)$} (0.75,1.5);
  % \draw[dashed,shorten <=5pt] (-1.75,0) -- node[below,yshift=15pt,xshift=3pt]{$h_t^2 (\theta)$} (0.75,0.5);
  % \draw[dashed,shorten <=5pt] (-1.75,0) -- node[below]{$h_t^d (\theta)$} (0.75,-0.5);

  % \draw[<-,denselx dotted,rounded corners] (-0.375,-1) to (-0.375,-1.625) to node[above] {Conteyt $\theta$} (-2.25,-1.625);
\end{tikzpicture}
